A Comparative Study on Unsupervised Domain Adaptation Approaches for Coffee Crop Mapping

In this work, we investigate the application of existing unsupervised domain adaptation (UDA) approaches to the task of transferring knowledge between crop regions having different coffee patterns. Given a geographical region with fully mapped coffee plantations, we observe that this knowledge can be used to train a classifier and to map a new county with no need of samples indicated in the target region. Experimental results show that transferring knowledge via some UDA strategies performs better than just applying a classifier trained in a region to predict coffee crops in a new one. However, UDA methods may lead to negative transfer, which may indicate that domains are too different that transferring knowledge is not appropriate. We also verify that normalization affect significantly some UDA methods; we observe a meaningful complementary contribution between coffee crops data; and a visual behavior suggests an existent of a cluster of samples that are more likely to be drawn from a specific data.

==> GRSL - Template (Arxiv)/tex/Experiments.tex <==
%\section{Experimental Analysis}
\section{Methodology}

\iffalse
\begin{itemize}
	\color{red}
	\item Descrição do que será feito nessa seção, quais serão os experimentos feitos no artigo (provavelmente de 3 a 4): impacto da normalização de dados, existência da complementariedade de conhecimento entre os datasets, analise visual do impacto de modelos diferentes nas amostras dos datasets alvos (hipótese onde um dataset pode apresentar uma mistura de distribuições e modelos diferentes se adequam a distribuições diferentes);
\end{itemize}
\fi

We carried out an extensive set of experiments on a Brazilian Coffee Crops dataset in order to evaluate the robustness of UDA methods in a remote-sensing agriculture scenario.
The experiments were designed to answer the following research questions:

\begin{enumerate}
	\item Is UDA methods more effective than transferring without adaptation for coffee crop mapping? Which UDA approach is the most effective? When applied as a pre-processing step, how much does data normalization affect the quality of knowledge transfer?

	%\item Can knowledge transfer between coffee plantations datasets from different geographic regions yield satisfactory results?
	\item Can knowledge transfer between coffee plantations datasets from different geographic regions yield complementary results?

	\item Is it possible to infer a spatial relationship between coffee samples correctly predicted from learning models trained in different data sources?
	%\msa{I also don't get this question at all...}
	
	% Other option
	%\item When trained learning models in different data sources, it is possible to infer a spatial relationship between coffee samples correctly predicted?
	
	
\end{enumerate}

To answer question (1), we compare the selected UDA methods agaist a classifier with no adaptation strategy. We also compare the approaches by using the four most common ways to normalize data: L1-Norm, L2-Norm, L1-Norm followed by a Z-score standardize, and L2-Norm followed by a Z-score standardize. Although data pre-processing analysis is not always considered the main topic of analysis, different ways of normalizing the data before the adaptation phase can cause a great impact in the transference of knowledge.
%Concerning question (2), we used Venn diagrams to analyze the complementarity among predictions from different coffee datasets according to a tuple (normalization method, UDA approach).
Concerning question (2), we used Venn diagrams of predictions to analyze the complementarity among different coffee datasets according to a tuple (normalization method, UDA approach).
We selected the normalization method and UDA approach based on the most suitable tuple observed in the experiments conducted to answer question (1). 
%\msa{I also don't get what the previous sentence say. Venn diagrams of what?}
This experiment aims at investigating the contribution of knowledge from different sources to the same target data. Since domain shift can be caused by different latent aspects in remote sensing, it is expected that different sources will have complementary contributions in consideration for the same target data.
%\jef{A sentenca abaixo ainda pode ser melhorada. Nao estah muito clara}
%At last, to answer (3), we perform a visual analysis of samples which are correctly predicted by specific models, for the purpose of investigating a spatial relationship between predicted samples.
At last, to answer (3), we perform a visual analysis of samples which are correctly predicted by specific models, using two different methods to project the original representation of data in 2D-space: Principal Component Analysis and t-Distributed Stochastic Neighbor Embedding (TSNE).

%For this purpose, we propose a visual analysis of these samples using two different methods to project the original representation of data in 2D-space: Principal Component Analysis and t-Distributed Stochastic Neighbor Embedding (TSNE)


%At last to answer (3), we made a visual analysis of \note{over} the samples which are correctly predicted by specific models, for the purpose of investigating a spatial relationship between predicted samples.

%\sout{Firstly, we compare the baselines using four most common ways to normalize data in UDA: L1-Norm, L2-Norm, L1-Norm followed by a Z-score standardize, and L2-Norm followed by a Z-score standardize. 
%Although the pre-processing of data is usually a not focused topic, different ways of normalizing the data before of adaptation phase can cause a great impact in the transference of knowledge. Secondly, we select a pair (norm, baseline) which achieved the best results, regarding kappa metric and using a Venn diagram we analyze the complementary of predictions from different source data. The aim of this experiment is to inspect the contribution of acknowledgment from different sources for the same target data. Since the domain shift can be caused by different latent aspects in remote sensing, seems reasonable \note{is expected} that different sources will have complementary contributions in consideration for the same target data.\note{Insert datasets images?} Thirdly, a visual analysis was made of \note{over} the samples which are correctly predicted by specific models, for the purpose of investigating a spatial relationship between predicted samples.}



%%Datasets and codes will be available online on publication \footnote{URL}.
\subsection{Data}

\iffalse
\begin{itemize}
	\color{red}
	\item Descrição dos dados: Dataset em geral, como foi balanceado e o descritor utilizado para representação computacional.
\end{itemize}
\fi

%As a focus of our work, we propose an evaluation in an agricultural scenario due to the challenges previously \note{optional or before} mentioned in Section \ref{intro}.\note{Optional Phrase} 
The Brazilian Coffee Scenes~\footnote{\url{ http://www.patreo.dcc.ufmg.br/2017/11/12/brazilian-coffee-scenes-dataset/}} dataset consists of \note{comprises} four remote sensing images composed of multi-spectral scenes taken by the SPOT sensor in 2005, covering regions of coffee cultivation over four counties in the state of Minas Gerais, Brazil: Arceburgo (AR), Guaxup\'{e} (GX), Guaran\'{e}sia (GA) and Monte Santo (MS). Each county is partitioned into multiple tiles of 64 x 64 pixels, which are divided into 2 classes (coffee and non-coffee). To mitigate the problem of imbalanced datasets (which is an issue corresponding to the significant difference\note{disparity or discrepancy} among the number of samples in the different classes) we applied a random under-sampling technique, balancing the data by randomly selecting a subset of data for the targeted classes.
%We use each source of images as a domain, consequently we get four domains (AR, GX, GA and MS) leading to 12 DA combinations.
In our analysis, we considered each county as a different domain, thus we have four domains (AR, GX, GA and MS) leading to 12 possible domain adaptation combinations.
%Considering each source of images as a domain, consequently \note{optional}, we get four domains (AR, GX, GA, and MS) leading to 12 DA combinations. As image representation we use a global low-level descriptor named Border/Interior Pixel Classification (BIC) \cite{stehling2002compact}.
%The BIC algorithm for classifying pixels in the border or interior basically \note{optional} separates the images into homogeneous and textured regions. Then, a color histogram is computed for each category of pixel. 
%A handmade descriptor was chosen over the deep representations due to the robustness show by authors \cite{nogueira2017towards} in the agricultural remote sensing scenario.
We have used a low-level descriptor named Border/Interior Pixel Classification (BIC) \cite{stehling2002compact} for feature extraction from coffee scenes. BIC is a very effective descriptor for coffee crops as shown in~\cite{nogueira2017towards,SantosPenattiTorres:visapp2010}.

%We employed a descriptor over the deep representations due to the robustness shown by authors \cite{nogueira2017towards} in the agricultural remote sensing scenario.

%We follow the standard protocol of [7, 8, 10, 14] for generating the source and target samples 1 .

\subsection{Setup and Implementation Details}

\iffalse
\begin{itemize}
\color{red}
\item Citar os baselines que foram utilizados e ja descritos na seções anteriores seguido das configurações dos experimentos (colocar o codigo todo online para reprodução cientifica)
\end{itemize}
\fi

We made a comparison between seven state-of-the-art methods: Transfer Component Analysis (TCA) \cite{pan2011domain}, Geodesic Flow Kernel (GFK) \cite{gong2012geodesic}, Subspace Alignment (SA) \cite{fernando2013unsupervised}, Joint Distribution Analysis (JDA) \cite{long2013transfer}, Transfer Joint Matching (TJM) \cite{long2014transfer}, CORAL \cite{sun2016return}, Joint Geometrical and Statistical Alignment (JGSA) \cite{zhang2017joint} and transfer with no adaptation (NA). A brief descriptions of methods is shown in Section \ref{related} (for more details we recommend the original papers).
%Usar no Related Work
% .TCA learns a set of transfer components in an RKHS such that when projecting domain data onto the latent space spanned by the transfer components, the distance between different distributions across domains is reduced and the variance is preserved as much as possible. 
% .GFK integrates an infinite number of subspaces that lie on the geodesic flow from the source subspace to the target one using the kernel trick. The flow represents incremental changes in geometric and statistical properties between the two domains. 
% .SA learn a linear transformation matrix M that maps the source subspace to the target one minimizing the Frobenius norm of their difference. In this way, the distance between different distributions across domains is reduced by moving closer the source and target subspaces exploiting the global covariance statistical structure of the two domains. 
% .JDA extends the Maximum Mean Discrepancy (MMD) to measure the difference in both marginal and conditional distributions (improving the TCA which consider only the marginal distribution) and integrate it with Principal Component Analysis (PCA) to create a feature representation that is effective and robust for substantial distribution difference \note{large domain shift}. 
% .TJM reduce the distribution difference between domains by jointly matching the features and reweighing the instances across domains in a principled dimensionality reduction procedure. 
% .CORAL aligns the distributions by re-coloring whitened source features with the covariance of the target distribution. 
% .JGSA reduces the domain shifts by taking both geometrical and statistical properties of source and target domain data into consideration and exploiting both shared and domain-specific features. To achieve that, an overall objective function is created by taking in account five terms: target variance, a variance between/within classes, distribution shift, and subspace shift.
We follow a full training evaluation protocol, where a Support Vector Machine (SVM) is trained on the labeled source data, and tested on the unlabeled target data. In our experimental setup, tuning of parameters is always made in the source data, since is impossible to use a cross-validation without labeled samples from the target domain.
We evaluate all methods by empirically searching the parameter space for optimal parameter settings that gives the highest average kappa on all datasets, and we report the best accuracy results of each method. 
%For subspace learning methods, we set the dimensions by searching k $\in$ [10, 20, . . . , 50]. Thus we use the remain free parameters recommended by the original papers.\note{Nao gostei dessa parte}



==> GRSL - Template (Arxiv)/tex/Introduction.tex <==
\section{Introduction}\label{intro}


% Remote sensing and coffee mapping
Accessibility to large sets of remote sensing images (RSIs) has increased over the years, and RSIs are currently a common source of information in many agribusiness applications.
Identifying crops is essential for knowing and monitoring land use, defining new land expansion strategies, and estimating viable production value.
In this work we focus on the use of RSIs for a crucial agro-economic activity in Brazil and, in particular, the state of Minas Gerais: the coffee crop mapping.

% Challenges in coffee crop recognition.
Automatic recognition of coffee plantations using RSIs is typically modeled as a supervised classification problem.
However, this task is rather challenging, mainly because the relief and age of the crop may hinder the recognition process,
Indeed, different spectral response and texture patterns can be observed for different regions.
For instance, coffee may grow in mountainous or in flat regions (as in Brazilian cerrado-savannas), and mountains may introduce shadows and distortions in the spectral information, making the corresponding patterns appear very different from those of coffee grown in flat geographic regions. 
Because of this, spectral information may be significantly reduced or even totally lost. 
Moreover, since the growing of coffee is not a seasonal activity, there may be coffee plantations of different ages in different regions, which also affects the observed spectral patterns.

% O problema da obtenção de amostras rotuladas
Although several approaches have advanced the state of the art in mapping coffee in recent years~\cite{SantosPenattiTorres:visapp2010,Nogueira2015:CIARP,nogueira2017towards}, one problem still remains: how to obtain representative samples for classification of new geographic areas of study?
%The size and quality of the training set have a direct impact on the execution time needed for training and on the final result of the classification. But the main issue is that 
The first possible strategy is the labeling of new samples, but it usually depends on experts, and even for them, it is not always possible to visually identify the patterns in the images. Thus, 
this process often requires visits to the study site, which can add extra costs to the analysis.
An alternative strategy to obtain extra data for training models is to transfer knowledge from already mapped regions. However, as Nogueira et al.~\cite{Nogueira2015:CIARP} has shown, due to the aforementioned differences that may exist in the coffee patterns between different geographic regions, direct transfer does not result in satisfactory quality.

% Objectives
In this work we investigate the application of existing unsupervised domain adaptation (UDA) approaches to the task of transferring knowledge from between crop regions having different coffee patterns. Our intent is to evaluate the effectiveness of UDA approaches to map new coffee crop areas.
% Motivation to study UDA
UDA methods allow labeled data to be employed from one or more prior datasets with the aim of create a learning model for unseen or unlabeled data. As assumption of UDA, the source (prior labeled datasets) and target (new unlabeled data) domain have related but different probability distributions, and the divergence between such distributions is called \emph{domain shift}.
This phenomenon can arise in several visual applications, caused, for instance, by human pose-changes in estimation tasks, luminosity variations in photos, differences in acquisition sensors, or the use of multi-view descriptions of a same object (draw, sketch, photo, textual description). 

Since supervised learning methods typically expect both source and target data to follow a same distribution, the presence of domain shift can degrade the accuracy on target data if the training occurs directly in a source domain without a proper domain adaptation, i.e., a correction of the difference between source and target distributions.
Ideally, we would like to learn a proper domain adaptation in an unsupervised manner.
The task, however, is rather challenging, and its relation with realistic applications has been drawing attention in last years~\cite{zhangtransfer}.
% Negative Transfer 
%\ede{Most current work focuses on ``What to transfer'' and ``How to transfer'', by implicitly assuming that the source and target domains be related to each other. However ``When to transfer'' is the most challenging topic, that asks in which situations transferring skills should be done. In the worst case, Transfer Learning may even hurt the performance of learning only in the target domain, a situation which is often referred to as Negative Transfer. How to avoid Negative Transfer is an important open issue even that is attracting more and more attention in the future \cite{ball2017comprehensive}. Thus, how to make sure that no negative transfer happens is a crucial issue \cite{pan2010survey} in transfer learning.}
% End conclusion
%To summarize, the main contribution of this work is an approach capable of combining different modalities of sensor data by using the inherent feature selection of the boosting- based strategy. This paper is organized as follows: Section II is an overview of the current multi-source remote sensing data fusion tech- niques. Section III presents details of the proposed approach. Section IV shows the corresponding evaluation protocol and experimental results of the proposed method. We conclude this work in Section V with some remarks and the future directions in the research.
Encouraged by these challenges, in this paper we perform a comparative experimental study of various methods for UDA in a specific view of remote sensing data. We use the dataset composed by four remote sensing images of coffee crop agriculture in scenarios with different plant and terrain conditions. 
%We analyze the eight UDA approach according to through empirical studies using different ways to normalize data, inspecting the visual behavior and complementarity over the final predictions.

This paper is organized as follows: Section II presents an overview of UDA techniques. Section III and IV presents, respectivelly, the evaluation protocol and experimental results of our analysis. We conclude this work in Section V with some remarks and the future directions in the research.





==> GRSL - Template (Arxiv)/tex/Introduction_edemir.tex <==
\section{Introduction}\label{intro}

\iffalse
\begin{itemize}
	\color{red}
	\item Grande quantidade de dados provenientes de sensores são gerados levando a uma grande quantidade de dados a serem analisados.
	
	\item Apesar da quantidade de dados gerados, a escassez de dados rotulados ainda é um problema principalmente nas abordagens de visão computacional onde se é usado a aprendizagem supervisionada
		
	\item Para contornar esse caso, a adaptação de domínio não supervisionada é usada.
	
	\item Uma das grandes motivações em relação a adaptação de domínio é na área de sensoriamento remoto (discursar o porque em sensoriamento remoto a adaptação de domínio é muito importante)
	
	\item O que foi está sendo proposto no paper, como isso foi feito e a descrição das próximas seções.
\end{itemize}

\fi

%The introduction should briefly place the study in a broad context and highlight why it is important. It should define the purpose of the work and its significance.
%\jef{Frase començando com verbo? Quem ``aumentou''? REESCREVER!}

%Over the years, there has increased significantly \note{optional} the number of remote sensing images availability.
%This was possible thanks to a new generation of satellite missions with short revisit time, as well the popular commercialization of drone-mounted cameras~\cite{tuia2016domain}.
The accessibility to large sets of remote sensing images has increased over the years. The main reasons are a new generation of satellite missions with short revisit time, as well as the popularization of drone mounted cameras.

Despite the extensive quantity of unlabeled data for visual analysis, a lack of labeled data is still a problem for some applications in remote sensing. This normally happens because of the difficult to acquire or create labeled sets. For example, in agriculture is common to send specialists to the field to collect and identify the data. Considering that a large scale plantation can cover hundreds of kilometers, a manual inspection over the area can last more than months and be finishing obtaining annotations \note{data} with a difference of dates. Another obstacle is the bad accessibility of the interested region. Depending on the application, is expensive or even impossible to recollect the required labeled data and rebuild learning models for every new task. Since the annotated data is essential for a good performance of supervised learning methods, alternative ways are explored.

%\note{Desenvolver o problema de falta de dados anotados: ;como isso pode afetar; como é feito atualmente, ; porque isso é um problema}
To surpass the problem, several approaches were developed in the last years, exploiting unlabeled data in concern of unsupervised domain adaptation (UDA). In this manner, labeled data can be employed from one or more prior datasets with the aim of create a learning model for unseen or unlabeled data.
%\jef{SIM! O que é adaptação de domínio? Como isso pode ajudar a solucionar o problema que você mencionou? Minha sugestão é você discutir do ponto de vista conceitual que bases de conhecimento já existentes podem formar uma rede. Talvez seja interessante criar uma figura.}
%In general, the \note{The} unsupervised domain adaptation problem takes advantage of labeled data in one or more source domains with the objective \note{aim} of create a learning model for unseen or unlabeled data in a target domain.
% Essa parte ficou complexa e confusa.
%However, domain adaptation has the main assumption that exists an affinity between a source and target domains, but strong enough to differ from a supervised learning problem where both data originate from the same distribution. 
%In other words, when \note{When} the assumption of domain adaptation is satisfied, the source and target domain distributions have related but different distributions
When the assumption of UDA is satisfied, the source (prior labeled datasets) and target (new unlabeled interested data) domain have related but different probability distributions and such divergence is named as \emph{domain shift}.
Such phenomenon can be seen in several visual applications. For example, human pose changes in estimation task, a variation of luminosity in photos, differences in acquisition sensor, multi-view descriptions of the same object (draw, sketch, photo, textual description) etc.

% Optional
%Domain shift is also present in remote sensing context, as can be seen in Figure \ref{domain_shift}.

Since supervised learning methods expect that both data follow the same distribution, domain shift can degrade the performance on target if trained directly in a source domain without a correct adaptation. In view of the challenges proposed by unsupervised domain adaptation, this research field has been drawing attention in last years due to the realistic proposed scenarios~\cite{zhangtransfer}.

%One major motivation of this paper is to handle with domain adaptation of agriculture images.
The main motivation of this letter is to handle with domain adaptation for agriculture scenarios. More specifically, we are interested in mapping coffee crops across different geographic domains, i.e., we want to evaluate if existing UDA methods are effective in scenarios with plant variations and terrain conditions. Although the use of remote sensing is crucial, the monitoring of agricultural activities shows unique challenges regarding the others computer vision applications. For instance, the coffee production follows strong seasonal patterns related to the biological life-cycle of crops. In addition, it depends on the physical landscape (e.g. soil type, elevation, etc) as well \note{and} their climatic driving variables due to the relationships with photo-period, fruits removal, photosynthesis and agricultural management practices \cite{atzberger2013advances}. Since the data is highly \note{optional} variable in space and time, a domain shift is clearly \note{optional} notable and a great effort is required to identify and make a transference of knowledge between a labeled source data to an unlabeled target domain. 

%\jef{Esse paragrafo esta meio estranho. Sugiro reescrever pra deixar a ideia mais clara.}
Unsupervised domain adaptation draw attention particularly for remote-sensing expecialists. In this field is common provide particular solutions for every new mapping and detection task. Avoiding discart labeled images available from a similar task and adapt to improve a new remote sensing task is highly desired.
%\sout{Furthermore, remote-sensing experts are exclusively interested in domain adaptation since it is common to provide particular solutions for detection/mapping tasks, discarding the previous solutions. In addition, is ignored the fact that multiple images available from a similar task could be adapted to improve a new remote sensing task.} 
However, as showed by authors in \cite{zhao2017multiple} the performance on a target domain depends on the worst empirical error among multiple source domains. So an insertion of non adaptive data without an adequate adaptation can degrade a final learning model or lead to suboptimal solutions.

%However, in many application scenarios, the labeled data available may come from multiple domains with different distributions. As a result, naive application of the single-source-single-target DA algorithms may lead to suboptimal solutions. Such problem calls for an efficient technique for multiple source domain adaptation.

%\jef{Acho que da pra reescrever e reduzir esse paragrafo pela metade.}

Encouraged by these challenges, in this paper we propose a comparative experimental study of various methods for UDA in a specific view of remote sensing data. To evaluate, we use the dataset, Brazilian Coffee Crops, that contains four remote sensing images of coffee crop agriculture in scenarios with plant variations and terrain conditions. We analyze the 7 methods through empirical studies using different ways to normalize data, inspecting the visual behavior and complementarity over the final predictions.

%In our experiments, firstly \note{optional} we study the most commons normalization methods for data processing. Thereafter, we propose an analysis of predictions from different adaptation methods and shown the complementary acknowledgment extracted from various approaches. At last a visual study was made over the samples corrected predicted from different adaptation methods, projecting in a 2D-space using two visualization approaches.

%\sout{Encouraged by these challenges, in this paper we propose a comparative experimental study of various methods for unsupervised domain adaptation in a specific view of remote sensing data. In order to \note{To} evaluate,  we use the dataset, Brazilian Coffee Crops, that contains \note{has} four remote sensing images of coffee crop agriculture in different geolocation \note{spatial context}. In our experiments, firstly \note{optional} we study the most commons normalization methods for data processing. Thereafter, we propose an analysis of predictions from different adaptation methods and shown the complementary acknowledgment extracted from various approaches. At last a visual study was made over the samples corrected predicted from different adaptation methods, projecting in a 2D-space using two visualization approaches.}


==> GRSL - Template (Arxiv)/tex/RelatedWork.tex <==



%\section{Related Work}\label{related}
\section{Unsupervised Domain Adaptation Approaches}\label{related}

UDA methods can be organized in three main categories \cite{zhangtransfer}: 
(1) instance-based, (2) feature-based, and (3) classifier-based. 
%All methods above rely on different properties, covering separates challenges in UDA. 

In instance-based adaptation is re-weight data in the source domain or in both domains to reduce domain divergence. In feature representation is attempt to learn a new feature representations to minimize \note{decrease} domain shift and error of learning task. In classifier-based is learn a new model that minimizes the generalization error in the target domain via training instances from both domains.
%Since labeled data in the target domain is not available in unsupervised domain adaptation, the classifier-based adaptation is unfeasible.
%Regarding the literature, domain adaptation can be divided into three main categories of knowledge would be transferred: instance-based adaptation (re-weight some \note{optional} data in the source domain or in both domains to reduce domain divergence), feature representation adaptation (learn a new feature representations to minimize \note{decrease} domain shift and error of learning task), and classifier-based adaptation (learn a new model that minimizes the generalization error in the target domain via training instances from both domains) \cite{zhangtransfer}. Since labeled data in the target domain is not available in unsupervised domain adaptation, the classifier-based adaptation is unfeasible.

In this work, we focused on feature-based UDA methods. Seven approaches were selected from the literature and are summarized in Table~\ref{properties} according to their main properties. Note that they are grouped into three branches: Data-centric, Subspace centric, and Hybrid methods. We breafly introduce each UDA method according to their branch in the next subsections.

\begin{table}[h!]
	\centering
	\caption{Summary of Unsupervised Domain Adaptation Methods}
	\label{properties}
	\tabcolsep=0.075cm
	\scalebox{0.85}
	{
		\begin{tabular}{llccccc}
			\hline
			& Approaches & \begin{tabular}[c]{@{}c@{}}Preserve\\ Variance\end{tabular} & \begin{tabular}[c]{@{}c@{}}Marginal\\ Distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Conditional\\ Distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Reweight\\ Instances\end{tabular} & \begin{tabular}[c]{@{}c@{}}Geometric\\ Structure\end{tabular} \\ \hline
			\multirow{3}{*}{Data Centric} & TCA~\cite{pan2011domain} & \checkmark & \checkmark &  &  &  \\
			& JDA~\cite{long2013transfer} & \checkmark & \checkmark & \checkmark &  &  \\
			& TJM~\cite{long2014transfer} & \checkmark & \checkmark &  & \checkmark &  \\ \hline
			\multirow{2}{*}{Subspace Centric} & SA~\cite{fernando2013unsupervised} & \checkmark &  &  &  &  \\
			& GFK~\cite{gong2012geodesic} & \checkmark &  &  &  & \checkmark \\ \hline
			\multirow{2}{*}{Hybrid} & CORAL~\cite{sun2016return} & \checkmark &  &  &  & \checkmark \\
			& JGSA~\cite{zhang2017joint} & \checkmark & \checkmark &  & \checkmark & \checkmark \\ \hline
		\end{tabular}
	}
\end{table}



\subsection{Data centric Approaches}

To align source and target data, data-centric methods attempt to find a specific transformation that can project both domains into a domain-invariant space. The distributional divergence between domains is reduced, while preserving the data properties from the original spaces~\cite{pan2011domain,long2013transfer,long2014transfer}. 
%The methods in \cite{pan2011domain}, \cite{long2013transfer} and \cite{long2014transfer} are examples of data-centric approaches.

\noindent \textbf{Transfer Component Analysis (TCA)}~\cite{pan2011domain}: its goal is to learn a set of transfer components in a Reproducing Kernel Hilbert Space.
When projecting domain data onto the latent space spanned by the transfer components, the distance between different distributions across domains is reduced while variance is preserved.% as much as possible.


%In \cite{pan2011domain}, the authors propose a method called \textbf{Transfer Component Analysis (TCA)}, whose goal is to learn a set of transfer components in a Reproducing Kernel Hilbert Space. When projecting domain data onto the latent space spanned by the transfer components, the distance between different distributions across domains is reduced while variance is preserved.% as much as possible.

%Due to several external factors and noise in observation data is reliable to state that $P_s(X_s) \ne P_t(X_t)$, however TCA rely in a claim that exists a transformation $\phi$ such that $P(\phi(X_s)) \approx P(\phi(X_t))$ and $P(Y_s|\phi(X_s)) \approx P(Y_t|\phi(X_t))$. Then without the labeled data from target domain, TCA learn the transformation function $\phi$ such that: minimize the marginal distribution between $P(\phi(X_s))$ and $P(\phi(X_t))$ and preserve the variance information of the original source $X_s$ and target $X_t$ data. The both requirements remark as important for a classification task, and the Fig \ref{tca} shows solid disadvantages when these features are optimized apart.

%
%\begin{figure*}[!ht]
%	\centering
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/A.pdf}
%		\label{fig:A}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/C.pdf}
%		\label{fig:C}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/B.pdf}
%		\label{fig:B}
%	}
	
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/D.pdf}
%		\label{fig:D}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/E.pdf}
%		\label{fig:E}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/F.pdf}
%		\label{fig:F}
%	}
%	\caption{Importance of simultaneous optimization considering the distance of distributions and preserving the maximum variance. In \textbf{(a)} the source and target domain are clearly apart each other. Minimizing the distance between domains projecting the data over the axis $X_2$ \textbf{(b)} result in a mixture of classes degrading classification performance. However projecting the data in axis $X_1$ \textbf{(c)}, preserve variance and result in a better separability for a classification task. On the other hand, considerer the source and target domain in \textbf{(d)}. Minimizing the distance between domains in \textbf{(d)}, projecting in $X_2$ axis \textbf{(f)}, creates a good separability. While preserving the variance in $X_1$ \textbf{(e)} axis, mix and reduce discrimination of classes.}

	%\caption{Importance of simultaneous optimization considering the distance of distributions and preserving the maximum variance. In \textbf{(a)} the source and target domain are clearly apart each other. However minimizing the distance between domains projecting the data over the axis $X_2$ \textbf{(b)} result in a mixture of classes degrading classification performance, while projecting the data in axis $X_1$ \textbf{(c)}, preserve variance, result in a better separability for a classification task. On the other hand, minimizing \note{Minimizing} the distance between domains in \textbf{(d)}, projecting in $X_2$ axis \textbf{(f)}, creates a good separability while preserving the variance in $X_1$ \textbf{(e)} axis, mix and reduce discrimination of classes.}
	%Minimizing distance between marginal distributions. \textbf{(b)} Maximizing Variance.}
%	\label{tca}
%\end{figure*}


\noindent \textbf{Joint Distribution Adaptation (JDA)}~\cite{long2013transfer}: it extends the Maximum Mean Discrepancy to measure the difference in both marginal and conditional distributions. Despite minimizing the marginal distribution between the source and target data, TCA does not guarantee that conditional distributions are reduced in this formulation, which may lead to a poor adaptation. JDA improves TCA, and integrates Maximum Mean Discrepancy with Principal Component Analysis to create a feature representation that is effective and robust for large domain shifts. 

%Despite minimizing the marginal distribution between the source and target data, TCA does not
%guarantee that conditional distributions are reduced in this formulation, which may lead to a poor adaptation. To \note{In order to} handle this problem, Mingsheng et al. \cite{long2013transfer} proposed a method called \textbf{Joint Distribution Adaptation (JDA)}, which extends the Maximum Mean Discrepancy to measure the difference in both marginal and conditional distributions. In this way, JDA improves TCA, and integrates it with Principal Component Analysis to create a feature representation that is effective and robust for large domain shifts. 

%Despite TCA minimize the marginal distribution between the source and target data, the conditional distributions are not guaranteed explicit reduced in this formulation, that could lead to a poor adaptation. In order to \note{To} handle this problem, Mingsheng et al. \cite{long2013transfer} proposed a method called Joint Distribution Adaptation (JDA) which extends the Maximum Mean Discrepancy (MMD) to measure the difference in both marginal and conditional distributions (improving the TCA which consider only the marginal distribution), and integrate it with Principal Component Analysis (PCA) to create a feature representation that is effective and robust for substantial distribution difference \note{large domain shift}. To achieve this, JDA proposes a transformation T where the joint expectations of features \textbf{x} and labels \textbf{y} are matched between domains using as follows:
%\begin{equation}
%\begin{split}
%& \underset{T}{min} ||\mathbb{E}_{P(x_s, y_s)}[T(x_s), y_s] - %\mathbb{E}_{P(x_t, y_t)}[T(x_t), y_t] ||^{2} \approx \\ & %||\mathbb{E}_{P_s(x_s)}[T(x_s)] - %\mathbb{E}_{P_t(x_t)}[T(x_t)] ||^{2} + \\ & %||\mathbb{E}_{P_s(y_s|x_s)}[y_s|T(x_s)] - %\mathbb{E}_{P_t(y_t|x_t)}[y_t|T(x_t)] ||^{2}
%\end{split}
%\end{equation}
%However, since the labels in target data are not available in unsupervised domain adaptation, the $P_t(y_t|x_t)$ cannot be estimated directly. Thus JDA assumes that $P_t(y_t|x_t) \approx P_s(y_t|x_t) $ and explore the sufficient statistics of conditional distributions $P_s(x_s|y_s)$ and $P_t(x_t|y_t)$.
%where is used pseudo labels of the target data by using the predictions of a base learning model trained in source data and testing in target data.


%A visual example is showed in Figure \ref{tjm}.
%\begin{figure}[]
%	\centering
%	\subfloat[Aligned domains - All samples]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/Teste_Var.pdf}
%		\label{fig:Teste_Var}
%	}
%	\subfloat[Aligned domains - Relevant Samples]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/Teste_Var_2.pdf}
%		\label{fig:Teste_Var_2}
%	}
%	\label{fig:reweight}
%	\caption{The relevance of instances after a domain adaptation. An example of a source and target domains aligned is showed in \textbf{(a)}. Despite the good alignment, there is a set of samples inside the ellipse which seems to be more relevant than others (fig \textbf{b}) which recalls as outliers. Depending on learning model, irrelevant/noise samples can degrade final adaptation model highlighting the importance of reweighing the samples by their importance.}
%	\label{tjm}
%\end{figure}

\noindent\textbf{Transfer Joint Matching (TJM)}~\cite{long2014transfer} aims at minimizing the distribution distance between domains trying to properly reweigh the instances which are more valuable to a classification task in the final adaptation. 
It is important because some instances from source data could have more relevance for classification task than others due to the huge difference of initial data representation.


%To that end, a new method named \textbf{Transfer Joint Matching (TJM)} was proposed by Long et al.~\cite{long2014transfer}. The main objective \note{aim, goal} of TJM beyond minimizing the distribution distance between domains is trying to properly reweigh the instances which are more valuable to a classification task in the final adaptation. 

%The Fig \ref{tjm} represents \note{is} a good example \note{intuition} of how two distributions even when adapted and aligned can show a significant difference in feature space. 
%This behavior can be exploited by focusing and reweighing the samples which are \note{optional} relevant for the adaptation. 
%Thus TJM in a two-step algorithm creates a transformation matrix T which reduce the distance of domains and reweigh the source samples to force a sparse structure between samples (Eq. \ref{tjm_opt)}).

%\begin{equation}\label{tjm_opt}
%\resizebox{\columnwidth}{!}
%{
%$\underset{T}{min} ||\mathbb{E}_{P(x_s)}[T(x_s)] - \mathbb{E}_{P(x_t)}[T(x_t)] ||^{2} + \lambda ||T||_{2,1}$
%}
%\end{equation}

%In TJM the marginal distribution is minimized through a feature matching in RKHS, as the same way of JDA, but for the reweighing of samples the authors proposed to incorporate an instance regularization in the problem formulation to force sparsity and assist in the final adaptation.

%in the transformation matrix A from Kernel-PCA, to assist in the final adaptation (Eq. \ref{sparsity}).

%\begin{equation}
%\resizebox{\columnwidth}{!}
%{
%${Sparsity~Regularization:~}
%||A_{s}||_{2,1} + ||A_{t}||_{F}^2$
%}
%\end{equation}\label{sparsity}

%Despite all mentioned methods assert that a good feature representation has to be capable of minimize the difference of distributions between domains \note{decrease the domain shift} as much as possible preserving the original properties, these methods fall in an assumption that there exists a transformation function which can project the source and target data into a common subspace which reduce the distribution difference between them and keep preserving some \note{optional} original information. Problems which a not too strongly related data \note{weak related}, i.e. strong domain shifts, can suggest that is may not exist such a space which preserve original properties and minimize in an optimal way \note{optimally} the distribution distance.

%Despite all mentioned methods assert that a good feature representation has to be capable of minimize the difference of distributions between domains \note{decrease the domain shift} as much as possible preserving the original properties, 

TCA, JDA, and TJM rely on the assumption that there always exists a transformation function which can project the source and target data into a common subspace which, at the same time, reduce distribution difference and preserves most original information. This assumption, however, is not realistic: known problems arising from strong domain shifts suggest that there may not always exist such a space.

%Advantages of data centrics


%Disvantages of data centrics

%--However, these methods require a strong assumption that there exist a unified transformation to map source and target domains into a shared subspace with small distribution shift. [At the same time preserving the information (geometric, statistics) of the original data]

%The data centric methods only exploit shared feature in two domains, which will fail when the two different domains have large discrepancy, because there may not exist such a common space where the distributions of two domains are the same and the data properties are also maximumly preserved in the mean time.


\subsection{Subspace Centric Approaches}

In contrast to data-centric methods, subspace-centric methods do not assume the existence of a unified transformation. They rely on a subspace manipulation of the source and target domains \cite{fernando2013unsupervised} or between them \cite{gong2012geodesic}, upholding that separate subspaces have very \note{optional} particular features to be exploited.

\noindent\textbf{Subspace Alignment (SA)}\cite{fernando2013unsupervised}: it projects source and target data onto different subspaces using PCA as a robust representation.
The method, then, learns a linear transformation matrix $M$ that aligns the source subspace to the target one while minimizing the Frobenius norm of their difference. In this way, the distance between different distributions across domains is reduced by moving closer the source and target subspaces exploiting the global covariance statistical structure of the two domains. 

% Fernando et al. \cite{fernando2013unsupervised} propose a \textbf{Subspace Alignment (SA)} method that projects source and target data onto different subspaces using PCA as a robust representation.
%The method, then, learns a linear transformation matrix $M$ that aligns the source subspace to the target one while minimizing the Frobenius norm of their difference. In this way, the distance between different distributions across domains is reduced by moving closer the source and target subspaces exploiting the global covariance statistical structure of the two domains. 

%As an alternative to SA, Gong et al.~\cite{gong2012geodesic} propose an extension of the work by Gopalan et al. \cite{gopalan2011domain}, taking advantage of Grassmannian manifold. 
%In geometric definition, a Grassmannian $\mathbb{G}$(d,V) is a collection of all d-dimensional subspaces of the n-dimensional vector space V. 
%In view of domain adaptation the computed subspaces from source and target domain are mapped each one into a point in Grassmannian manifold. As pointed in \cite{gong2012geodesic}, the distance between two points in Grassmannian manifold can represent how similar the original projections are regarding their marginal distribution. %For example, consider the problem of knowledge transfer between two datasets of coffee crop in different regions of a country. The highly variable of these data, when projected into a Grassmannian manifold, will result in points far apart from each other. 
%However, the geodesic curve between these points represents intermediate subspaces which can carry some \note{optional} variant geometric and statistics properties that state a relationship between the two domains. Capture and use the largest number of subspaces as possible may help to extract the necessary information to make an effective domain adaptation.
%In \cite{gopalan2011domain} the authors explore the geodesic flow curve connecting the source and target domain on the Grassmannian manifold, sampling a discrete number of subspaces as representations and concatenation them into a feature vector for learning purpose. 

\noindent \textbf{Geodesic Flow Kernel (GFK)}\cite{gong2012geodesic}: is an elegant approach that integrates an infinite number of subspaces that lie on the geodesic flow from the source subspace to the target one using the kernel trick.
%, thereby overcoming some drawbacks in the original approach. 
The main drawback of subspace-centric methods is that, while focused in reducing the geometrical shift between subspaces, the distribution shift between projected data of domains is not explicitly treated as in data-centric methods.
Moreover, the subspace dimension to project the data normally requires some tuning of parameters or preprocessing, which can be computationally expensive.


%However, Gong et al. proposed the \textbf{Geodesic Flow Kernel (GFK)} as an elegant approach that integrates an infinite number of subspaces that lie on the geodesic flow from the source subspace to the target one using the kernel trick, thereby overcoming some drawbacks in the original approach. The main drawback of subspace-centric methods is that, while focused in reducing the geometrical shift between subspaces, the distribution shift between projected data of domains is not explicitly treated as in data-centric methods.
%Moreover, the subspace dimension to project the data normally requires some tuning of parameters or preprocessing, which can be computationally expensive.

\subsection{Hybrid Approaches}

\noindent\textbf{CORAL}~\cite{sun2016return}: it was proposed to tackle the drawbacks of data and subspace-centric methods. In this approach, the domain shift is minimized by aligning the covariance of a source and target distributions in the original data.
%More recently, to tackle the drawbacks of data and subspace-centric methods, Sun et al. \cite{sun2016return} propose the \textbf{CORAL} adaptation. In this approach, the domain shift is minimized by aligning the covariance of a source and target distributions in the original data.
%For this purpose CORAL can be divided into two simple steps: 1) computation of the covariance matrices of the source and target data; 2) applying the whitening and re-coloring linear transformation only to the source features.
In contrast to subspace-centric methods, CORAL suggests an alignment without the need of subspace projection, which would require intense computation and complex hyper-parameter tuning. 
%Regarding the authors, these methods commonly \note{optional} align only the bases of subspaces, not considering the distribution of project data. 
In addition, CORAL do not assume a unified transformation like data-centric methods; it uses, instead, an asymmetric transformation only on source data. 

\noindent\textbf{Joint Geometric Subspace Alignment (JGSA)}~\cite{zhang2017joint}: it aims to reduce the statistical and geometrical divergence between domains using common and specific properties of the source and target data. To achieve that, an overall objective function is created by taking into account five terms: target variance, variance between/within classes, distribution shift, and subspace shift.

%To reach this objective JGSA tries to find two coupled projections A and B for source and target domain respectively that explore five different quantities together in a single objective function(Eq. \ref{jgsa}): 

%\begin{equation}
%\resizebox{\columnwidth}{!}
%{
%	$max \frac{\mu\{Target~Variance\} + \beta\{Between~Class~ Variance\} }{\{Distribution~Shift\} + \lambda\{Subspace~Shift\} + \beta\{Within~Class~Variance\}}	$
%}
%\label{jgsa}
%\end{equation}


%where $\mu$, $\lambda$, $\beta$, are regularization parameters used to handle with the trade-off of importance in every term of optimization. 

%As trying to address different drawbacks from data-centric and subspace centric, the run-time complexity of JGSA grows in comparison to the others methods since is needed to learn two different mapping projections. 

%All things considered, it seems \note{is} reasonable to assume that all methods rely on different properties covering separable challenges in UDA. Taking accounts these properties, a resume of challenges tackle for the methods is showed in Table \ref{properties}.




==> GRSL - Template (Arxiv)/tex/RelatedWork_edemir.tex <==

\iffalse
\section{Background Concepts}\label{background}


\begin{itemize}
	\color{red}
		
	\item Definição formal do problema UDA (Unsupervised Domain Adaptation): Domain, Task, Dataset, Problem
	
	\item Como o problema é ramificado de acordo com as abordagens dos artigos na literatura.(data centric e subspace centric)
	
	\item Discutir as vantagens e desvantagens de todos os baselines em uma linha cronológica em que eles foram propostos, e fazer uma tabela marcando as principais vantagens-desvantagens para ficar de fácil visualização.
	
\end{itemize}

In this work we follow the definitions proposed by Zhang et~al.~\cite{zhang2017cross} for ``domain'', ``task'' and ``dataset''.

\textit{Definition 1:} A \textbf{domain} is defined as $D = \{X, P(x)\}$, which is composed of two components: a feature space X and a marginal probability distribution $P(x)$, where $x \in X$ .

\textit{Definition 2:} Given a specific domain, a \textbf{task} is defined as $T = \{Y, f(x)\}$, which is composed of two components: a label space $Y$ and a predictive function $f(x)$, where $f(x)$ can be seen as a conditional distribution $P(y|x)$ and $y \in Y$.

\textit{Definition 3:} A \textbf{dataset} is defined as $S = \{X ,P(x), Y, f(x)\}$, which is a collection of data that belong to a specific domain with a specific task.

In unsupervised domain adaptation we assume that no labeled data is available in the target dataset, i.e., the labels of target dataset are unknown, but all \note{optional} unlabeled samples are available at training phase.

With the previous \note{earlier} definitions we can state the UDA problem:

\textit{Problem:} Given labeled source domain $D_s = \{(x_1 , y_1 ), ... , (x_{n_s} , y_{n_s} )\}$ and unlabeled target domain $D_t = \{x_{1}, ... , x_{n_t}\}$, where $n_s$ and $n_t$ are number of samples in source and target domain respectively, under the assumptions that: source and target domain share the same feature and label space  ($X_s = X_t, Y_s = Y_t$), and the samples from source and target domain are drawn from different distributions but related ($P_s(x_s) \neq P_t(x_t), P_s(y_s|x_s) \neq P_t(y_t | x_t)$). How to create a function h(.) that predicts the class label of a sample from the target domain $D_t$ using labeled source domain $D_s$ and unlabeled target domain $D_t$.


The main difference between supervised learning and UDA rely on the fact we have different but related distributions between source and target, making possible to make a transference of knowledge in order \note{optional} to reduce the distribution difference between domain.

\fi

%\section{Related Work}\label{related}
\section{Unsupervised Domain Adaptation Approaches}\label{related}

%Regarding the literature \cite{zhangtransfer}, 
\jef{Continua ruim. Leia essa frase: ``UDA can be divided into three main categories of knowledge would be transferred''. O que voce quis dizer?}

%According to the literature survey [21], existing domain adaptation methods can be roughly organized into two categories: feature matching and instance reweighting

\ede{Regarding the literature \cite{zhangtransfer}, UDA methods can be organized into tree main categories}: (1) instance-based, (2) feature-based and (3) classifier-based. In instance-based adaptation is re-weight some \note{optional} data in the source domain or in both domains to reduce domain divergence. In feature representation is attempt to learn a new feature representations to minimize \note{decrease} domain shift and error of learning task. In classifier-based is learn a new model that minimizes the generalization error in the target domain via training instances from both domains.
%Since labeled data in the target domain is not available in unsupervised domain adaptation, the classifier-based adaptation is unfeasible.
%Regarding the literature, domain adaptation can be divided into three main categories of knowledge would be transferred: instance-based adaptation (re-weight some \note{optional} data in the source domain or in both domains to reduce domain divergence), feature representation adaptation (learn a new feature representations to minimize \note{decrease} domain shift and error of learning task), and classifier-based adaptation (learn a new model that minimizes the generalization error in the target domain via training instances from both domains) \cite{zhangtransfer}. Since labeled data in the target domain is not available in unsupervised domain adaptation, the classifier-based adaptation is unfeasible.
In this work, we study methods based on a feature representation category, which can be divided into three branches: Data-centric, Subspace centric, and Hybrid methods.

\subsection{Data centric Approaches}

To align a source and target data, the data-centric methods attempt find a specific transformation that can project both domains into a domain invariant space. In this way is reduced the distributional divergence between domains and preserve the data properties in original spaces. The methods in \cite{pan2011domain}, \cite{long2013transfer} and \cite{long2014transfer} are examples of data-centric approaches. In \cite{pan2011domain}, the authors proposed a method called Transfer Component Analysis (TCA) which has as objective \note{aim} learn a set of transfer components in a Reproducing Kernel Hilbert Space. When projecting domain data onto the latent space spanned by the transfer components, the distance between different distributions across domains is reduced and the variance is preserved.% as much as possible.

%Due to several external factors and noise in observation data is reliable to state that $P_s(X_s) \ne P_t(X_t)$, however TCA rely in a claim that exists a transformation $\phi$ such that $P(\phi(X_s)) \approx P(\phi(X_t))$ and $P(Y_s|\phi(X_s)) \approx P(Y_t|\phi(X_t))$. Then without the labeled data from target domain, TCA learn the transformation function $\phi$ such that: minimize the marginal distribution between $P(\phi(X_s))$ and $P(\phi(X_t))$ and preserve the variance information of the original source $X_s$ and target $X_t$ data. The both requirements remark as important for a classification task, and the Fig \ref{tca} shows solid disadvantages when these features are optimized apart.

%
%\begin{figure*}[!ht]
%	\centering
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/A.pdf}
%		\label{fig:A}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/C.pdf}
%		\label{fig:C}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/B.pdf}
%		\label{fig:B}
%	}
	
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/D.pdf}
%		\label{fig:D}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/E.pdf}
%		\label{fig:E}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/F.pdf}
%		\label{fig:F}
%	}
%	\caption{Importance of simultaneous optimization considering the distance of distributions and preserving the maximum variance. In \textbf{(a)} the source and target domain are clearly apart each other. Minimizing the distance between domains projecting the data over the axis $X_2$ \textbf{(b)} result in a mixture of classes degrading classification performance. However projecting the data in axis $X_1$ \textbf{(c)}, preserve variance and result in a better separability for a classification task. On the other hand, considerer the source and target domain in \textbf{(d)}. Minimizing the distance between domains in \textbf{(d)}, projecting in $X_2$ axis \textbf{(f)}, creates a good separability. While preserving the variance in $X_1$ \textbf{(e)} axis, mix and reduce discrimination of classes.}

	%\caption{Importance of simultaneous optimization considering the distance of distributions and preserving the maximum variance. In \textbf{(a)} the source and target domain are clearly apart each other. However minimizing the distance between domains projecting the data over the axis $X_2$ \textbf{(b)} result in a mixture of classes degrading classification performance, while projecting the data in axis $X_1$ \textbf{(c)}, preserve variance, result in a better separability for a classification task. On the other hand, minimizing \note{Minimizing} the distance between domains in \textbf{(d)}, projecting in $X_2$ axis \textbf{(f)}, creates a good separability while preserving the variance in $X_1$ \textbf{(e)} axis, mix and reduce discrimination of classes.}
	%Minimizing distance between marginal distributions. \textbf{(b)} Maximizing Variance.}
%	\label{tca}
%\end{figure*}

Despite TCA minimize the marginal distribution between the source and target data, the conditional distributions are not guaranteed explicit reduced in this formulation, that could lead to a poor adaptation.  To \note{In order to} handle this problem, Mingsheng et al. \cite{long2013transfer} proposed a method called Joint Distribution Adaptation (JDA) which extends the Maximum Mean Discrepancy to measure the difference in both marginal and conditional distributions. In this way JDA improve TCA, which consider only the marginal distribution, and integrate it with Principal Component Analysis to create a feature representation that is effective and robust for a large domain shift. 

%Despite TCA minimize the marginal distribution between the source and target data, the conditional distributions are not guaranteed explicit reduced in this formulation, that could lead to a poor adaptation. In order to \note{To} handle this problem, Mingsheng et al. \cite{long2013transfer} proposed a method called Joint Distribution Adaptation (JDA) which extends the Maximum Mean Discrepancy (MMD) to measure the difference in both marginal and conditional distributions (improving the TCA which consider only the marginal distribution), and integrate it with Principal Component Analysis (PCA) to create a feature representation that is effective and robust for substantial distribution difference \note{large domain shift}. To achieve this, JDA proposes a transformation T where the joint expectations of features \textbf{x} and labels \textbf{y} are matched between domains using as follows:
%\begin{equation}
%\begin{split}
%& \underset{T}{min} ||\mathbb{E}_{P(x_s, y_s)}[T(x_s), y_s] - %\mathbb{E}_{P(x_t, y_t)}[T(x_t), y_t] ||^{2} \approx \\ & %||\mathbb{E}_{P_s(x_s)}[T(x_s)] - %\mathbb{E}_{P_t(x_t)}[T(x_t)] ||^{2} + \\ & %||\mathbb{E}_{P_s(y_s|x_s)}[y_s|T(x_s)] - %\mathbb{E}_{P_t(y_t|x_t)}[y_t|T(x_t)] ||^{2}
%\end{split}
%\end{equation}
%However, since the labels in target data are not available in unsupervised domain adaptation, the $P_t(y_t|x_t)$ cannot be estimated directly. Thus JDA assumes that $P_t(y_t|x_t) \approx P_s(y_t|x_t) $ and explore the sufficient statistics of conditional distributions $P_s(x_s|y_s)$ and $P_t(x_t|y_t)$.
%where is used pseudo labels of the target data by using the predictions of a base learning model trained in source data and testing in target data.
Even when distributions between domains are minimized, some instances from source data would have more relevance than others due to the huge difference of initial data. 

%A visual example is showed in Figure \ref{tjm}.
%\begin{figure}[]
%	\centering
%	\subfloat[Aligned domains - All samples]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/Teste_Var.pdf}
%		\label{fig:Teste_Var}
%	}
%	\subfloat[Aligned domains - Relevant Samples]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/Teste_Var_2.pdf}
%		\label{fig:Teste_Var_2}
%	}
%	\label{fig:reweight}
%	\caption{The relevance of instances after a domain adaptation. An example of a source and target domains aligned is showed in \textbf{(a)}. Despite the good alignment, there is a set of samples inside the ellipse which seems to be more relevant than others (fig \textbf{b}) which recalls as outliers. Depending on learning model, irrelevant/noise samples can degrade final adaptation model highlighting the importance of reweighing the samples by their importance.}
%	\label{tjm}
%\end{figure}
To that end, a new method named Transfer Joint Matching (TJM) was proposed by Long et al. \cite{long2014transfer}. The main objective \note{aim, goal} of TJM beyond minimizing the distribution distance between domains is trying to reweigh the instances which are more valuable to a classification task in the final adaptation. 

%The Fig \ref{tjm} represents \note{is} a good example \note{intuition} of how two distributions even when adapted and aligned can show a significant difference in feature space. 
%This behavior can be exploited by focusing and reweighing the samples which are \note{optional} relevant for the adaptation. 
%Thus TJM in a two-step algorithm creates a transformation matrix T which reduce the distance of domains and reweigh the source samples to force a sparse structure between samples (Eq. \ref{tjm_opt)}).

%\begin{equation}\label{tjm_opt}
%\resizebox{\columnwidth}{!}
%{
%$\underset{T}{min} ||\mathbb{E}_{P(x_s)}[T(x_s)] - \mathbb{E}_{P(x_t)}[T(x_t)] ||^{2} + \lambda ||T||_{2,1}$
%}
%\end{equation}

%In TJM the marginal distribution is minimized through a feature matching in RKHS, as the same way of JDA, but for the reweighing of samples the authors proposed to incorporate an instance regularization in the problem formulation to force sparsity and assist in the final adaptation.

%in the transformation matrix A from Kernel-PCA, to assist in the final adaptation (Eq. \ref{sparsity}).

%\begin{equation}
%\resizebox{\columnwidth}{!}
%{
%${Sparsity~Regularization:~}
%||A_{s}||_{2,1} + ||A_{t}||_{F}^2$
%}
%\end{equation}\label{sparsity}

%Despite all mentioned methods assert that a good feature representation has to be capable of minimize the difference of distributions between domains \note{decrease the domain shift} as much as possible preserving the original properties, these methods fall in an assumption that there exists a transformation function which can project the source and target data into a common subspace which reduce the distribution difference between them and keep preserving some \note{optional} original information. Problems which a not too strongly related data \note{weak related}, i.e. strong domain shifts, can suggest that is may not exist such a space which preserve original properties and minimize in an optimal way \note{optimally} the distribution distance.

%Despite all mentioned methods assert that a good feature representation has to be capable of minimize the difference of distributions between domains \note{decrease the domain shift} as much as possible preserving the original properties, 

These methods fall in an assumption that there exists a transformation function which can project the source and target data into a common subspace which reduce the distribution difference between them and keep preserving some \note{optional} original information. Problems with a strong domain shift suggest that is may not exist such a space which preserve original properties and minimize in an optimally the distribution distance.

%Advantages of data centrics


%Disvantages of data centrics

%--However, these methods require a strong assumption that there exist a unified transformation to map source and target domains into a shared subspace with small distribution shift. [At the same time preserving the information (geometric, statistics) of the original data]

%The data centric methods only exploit shared feature in two domains, which will fail when the two different domains have large discrepancy, because there may not exist such a common space where the distributions of two domains are the same and the data properties are also maximumly preserved in the mean time.

\subsection{Subspace Centric Approaches}

By contrast of data-centric, the subspace centric methods do not assume an existence of a unified transformation but rely on a subspace manipulation of the source and target domains \cite{fernando2013unsupervised} or between them \cite{gong2012geodesic}, upholding that separate subspaces have very \note{optional} particular features to be exploited. Fernando et al. \cite{fernando2013unsupervised} propose a Subspace Alignment (SA) method, which project source and target data to different subspaces using PCA as a robust representation and learn a linear transformation matrix M that align the source subspace to the target one minimizing the Frobenius norm of their difference. In this way, the distance between different distributions across domains is reduced by moving closer the source and target subspaces exploiting the global covariance statistical structure of the two domains. 

As an alternative of subspace alignment Gong et al. \cite{gong2012geodesic} proposes an extension of the work by Gopalan et al. \cite{gopalan2011domain}, taking advantage of Grassmannian manifold. 
%In geometric definition, a Grassmannian $\mathbb{G}$(d,V) is a collection of all d-dimensional subspaces of the n-dimensional vector space V. 
%In view of domain adaptation the computed subspaces from source and target domain are mapped each one into a point in Grassmannian manifold. As pointed in \cite{gong2012geodesic}, the distance between two points in Grassmannian manifold can represent how similar the original projections are regarding their marginal distribution. %For example, consider the problem of knowledge transfer between two datasets of coffee crop in different regions of a country. The highly variable of these data, when projected into a Grassmannian manifold, will result in points far apart from each other. 
%However, the geodesic curve between these points represents intermediate subspaces which can carry some \note{optional} variant geometric and statistics properties that state a relationship between the two domains. Capture and use the largest number of subspaces as possible may help to extract the necessary information to make an effective domain adaptation.
%In \cite{gopalan2011domain} the authors explore the geodesic flow curve connecting the source and target domain on the Grassmannian manifold, sampling a discrete number of subspaces as representations and concatenation them into a feature vector for learning purpose. 
However, Gong et al. proposed the Geodesic Flow Kernel (GFK) as an elegant approach that integrates an infinite number of subspaces that lie on the geodesic flow from the source subspace to the target one using the kernel trick, and overcoming some drawbacks in the original approach. The main drawback of subspace centric methods, while focused in reducing the geometrical shift between subspaces, the distribution shift between projected data of domains are not explicitly treated as in data-centric methods, and subspace dimension to project the data normally \note{optional} require some \note{optional} tuning of parameters or preprocessing.

\subsection{Hybrid Approaches}

More recent to overcome the drawbacks of data and subspace centric methods together, Sun et al. \cite{sun2016return} propose the CORAL adaptation. In this approach, the domain shift is minimized aligning the covariance of a source and target distributions in the original data.
%For this purpose CORAL can be divided into two simple steps: 1) computation of the covariance matrices of the source and target data; 2) applying the whitening and re-coloring linear transformation only to the source features.
In contrast to the subspace centric methods, CORAL suggests an alignment without a need of subspace projection, which requires an expensive computation and hyper-parameter tuning. 
%Regarding the authors, these methods commonly \note{optional} align only the bases of subspaces, not considering the distribution of project data. 
In addition, CORAL do not assume a unified transformation such as data-centric methods, instead, the method uses an asymmetric transformation only on source data. 

In \cite{zhang2017joint} Zhang et al. propose the Joint Geometric Subspace Alignment (JGSA) that aims to reduce the statistical and geometrical divergence between domains using the common and specific properties of the source and target data. To achieve that, an overall objective function is created by taking in account five terms: target variance, a variance between/within classes, distribution shift, and subspace shift.

%To reach this objective JGSA tries to find two coupled projections A and B for source and target domain respectively that explore five different quantities together in a single objective function(Eq. \ref{jgsa}): 

%\begin{equation}
%\resizebox{\columnwidth}{!}
%{
%	$max \frac{\mu\{Target~Variance\} + \beta\{Between~Class~ Variance\} }{\{Distribution~Shift\} + \lambda\{Subspace~Shift\} + \beta\{Within~Class~Variance\}}	$
%}
%\label{jgsa}
%\end{equation}


%where $\mu$, $\lambda$, $\beta$, are regularization parameters used to handle with the trade-off of importance in every term of optimization. 

%As trying to address different drawbacks from data-centric and subspace centric, the run-time complexity of JGSA grows in comparison to the others methods since is needed to learn two different mapping projections. 

%All things considered, it seems \note{is} reasonable to assume that all methods rely on different properties covering separable challenges in UDA. Taking accounts these properties, a resume of challenges tackle for the methods is showed in Table \ref{properties}.

All methods above rely on different properties, covering separates challenges in UDA. A summary of the properties considered for each method is shown in \ref{properties}

\begin{table}[h!]
	\centering
	\caption{Comparison of Approches Properties}
	\label{properties}
\tabcolsep=0.075cm
\scalebox{0.85}
{
	\begin{tabular}{ccccccc}
		\hline
		& Approches & \begin{tabular}[c]{@{}c@{}}Preserve\\ Variance\end{tabular} & \begin{tabular}[c]{@{}c@{}}Marginal\\ Distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Conditional\\ Distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Reweight\\ Instances\end{tabular} & \begin{tabular}[c]{@{}c@{}}Geometric\\ Structure\end{tabular} \\ \hline
		\multirow{3}{*}{Data Centric} & TCA & \checkmark & \checkmark &  &  &  \\
		& JDA & \checkmark & \checkmark & \checkmark &  &  \\
		& TJM & \checkmark & \checkmark &  & \checkmark &  \\ \hline
		\multirow{2}{*}{Subspace Centric} & SA & \checkmark &  &  &  &  \\
		& GFK & \checkmark &  &  &  & \checkmark \\ \hline
		\multirow{2}{*}{Hybrid} & CORAL & \checkmark &  &  &  & \checkmark \\
		& JGSA & \checkmark & \checkmark &  & \checkmark & \checkmark \\ \hline
	\end{tabular}
}
\end{table}


==> GRSL - Template (Arxiv)/tex/Results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Results and Discussion}
\iffalse
\begin{itemize}
	\color{red}
	\item Nessa seção são mostrados todos os experimentos realizados separados por subseções para cada experimento. Sempre a sequencia: o que foi feito, resultados, discussão.	
\end{itemize}
\fi

\subsection{UDA Approaches Comparison}

In this section, we compare different strategies of transferring knowledge between geographic domains in order to map coffee crops. 
We compared the SVM classifiers with no adaptation (NA) against the seven selected UDA approaches.
We also evaluated  four different way to normalize data over eight unsupervised domain adaptation approaches. In order to evaluate a normalization method, the mean accuracy value of all 12 UDA configuration was computed and reported. The mean accuracy results on each pair of counties from Brazilian Coffee Crops dataset are shown in Table \ref{tab_mean_acc}.

%The results on Brazilian Coffee Crops dataset are shown in Table \ref{tab5}.%\ref{tab1}, \ref{tab2}, \ref{tab3}, and \ref{tab4}.

%As can be seen, TCA achieved the higher performance over the baselines when using the L1 or L2 Norm followed by a Z-score standardize. SA and JGSA outperform the baselines solely using an L1 Norm and L2 Norm, respectively.
\begin{table}[]
	\centering
	\caption{Mean Accuracy of Methods using different Normalizations}
	\label{tab_mean_acc}
	\tabcolsep=0.155cm
	\begin{tabular}{ccccc}
		\hline
		Method & L1-Norm & L2-Norm & L1-Norm-Z-Score & L2-Norm-Z-Score \\ \hline
		NA     & 67,76   & 66,58   & 68,22           & 68,41           \\
		TCA    & 67,86   & 67,86   & \textbf{73,95}           & \textbf{74,31}           \\
		GFK    & 70,08   & 68,21   & 73,22           & 73,22           \\
		SA     & \textbf{72,80}   & 71,15   & 71,95           & 72,13           \\
		JDA    & 67,72   & 67,72   & 71,49           & 70,94           \\
		TJM    & 69,97   & 69,97   & 71,72           & 71,97           \\
		CORAL  & 64,85   & 65,38   & 71,67           & 70,94           \\
		JGSA   & 67,59   & \textbf{72,58}   & 70,18           & 70,02           \\ \hline
	\end{tabular}
\end{table}

The results show that, in general, it is better use some UDA strategy than try to transfer knowledge without no adaptation.
We can also observe that TCA achieved the best results in comparison with the other UDA approaches when using the L2 Norm followed by a Z-score standardize.
%\begin{table}[]
%	\centering
%	\caption{Mean Accuracy of Methods using different Normalizations}
%	\label{tab_mean_acc}
%	\tabcolsep=0.155cm
%	\begin{tabular}{ccccc}
%		\hline
%		Method & L1-Norm          & L2-Norm          & L1-Norm-Z-Score  & L2-Norm-Z-Score  \\ \hline
%		NA     & 67,7600          & 66,5841          & 68,2234          & 68,4066          \\
%		TCA    & 67,8606          & 67,8606          & \textbf{73,9479} & \textbf{74,3132} \\
%		GFK    & 70,0807          & 68,2115          & 73,2203          & 73,2203          \\
%		SA     & \textbf{72,8022} & 71,1538          & 71,9521          & 72,1333          \\
%		JDA    & 67,7196          & 67,7196          & 71,4873          & 70,9438          \\
%		TJM    & 69,9730          & 69,9730          & 71,7189          & 71,9706          \\
%		CORAL  & 64,8511          & 65,3767          & 71,6714          & 70,9408          \\
%		JGSA   & 67,5859          & \textbf{72,5836} & 70,1771          & 70,0247          \\ \hline
%	\end{tabular}
%\end{table}
%Despite the comparison of mean general results, it can be observed several remarkable points when the domain problems are views apart (separately):
%\msa{I don't get the previous sentence}
Despite the comparison of mean general results, it can be observed several remarkable points: 1) even though TCA achieving the best mean accuracy, the method had lower results in 9 of 12 combinations over the L2 Norm-Z-score setup, that could be a cost of an adaptation without taking into account the conditional distribution information; 2) the knowledge to be transferred between two domains is not always reciprocal, seems a case of JGSA which got the best results when trained at AR and test in MS but obtained the worst results when using MS to train and evaluate in AR.; 3) at the same setup mentioned before, in 3 of 12 combinations got the best results when none of the domain adaptations methods are used, that is 25\% of combinations had a negative transfer phenomenon. 
%Table \ref{tab5} shows a wider view of the cases of positive and negative transfer, i.e., the UDA approaches which got a better performance in comparison with a no adaptation approach are marked as blue, otherwise they are marked with red.
Table \ref{tab5} shows the cases of positive and negative transfer, where the UDA approaches which got a better performance in comparison with a no adaptation approach are marked as blue (Positive Transfer), otherwise they are marked with red (Negative Transfer).

%\msa{In fact, the whole previous paragraph is quite confusing and could use a thorough revision.}

\iffalse

\begin{table*}[]
	\centering
	\caption{Accuracy Using L1 Norm}
	\label{tab1}
	%\tabcolsep=0.06cm
	\scalebox{0.95}{
		\begin{tabular}{cccccccccccccc}
			\hline
			\begin{tabular}[c]{@{}c@{}}Method/\\ Src-Tgt\end{tabular} & AR-GX          & AR-GA          & AR-MS          & GX-AR          & GX-GA          & GX-MS          & GA-AR          & GA-GX          & GA-MS          & MS-AR          & MS-GX          & MS-GA          & Mean           \\ \hline
			NA       & 63,26          & 80,62          & 59,03          & 60,44          & 77,36          & 75,67          & 70,88          & 64,64          & 63,82          & 52,20          & 79,56          & 78,44          & 67,76          \\
			TCA      & 69,06          & 82,25          & 60,51          & 60,99          & 77,36          & 68,69          & 67,03          & 64,92          & 62,98          & 63,19          & 74,03          & 79,89          & 67,86          \\
			GFK      & 68,78          & 81,88          & 60,37          & 55,49          & 71,38          & 78,77          & \textbf{75,82} & 63,95          & 62,91          & 63,19          & \textbf{84,81} & 73,91          & 70,08          \\
			SA       & \textbf{70,86} & \textbf{83,88} & 59,73          & \textbf{72,53} & 77,17          & \textbf{79,76} & 73,08          & 64,09          & \textbf{64,39} & 63,19          & 84,67          & 77,54          & \textbf{72,80} \\
			JDA      & 69,89          & 82,07          & 60,08          & 61,54          & 77,36          & 68,41          & 67,03          & 66,85          & 63,19          & 65,38          & 73,90          & 79,71          & 67,72          \\
			TJM      & 70,17          & 80,80          & \textbf{61,00} & 71,43          & 78,44          & 68,12          & 69,78          & \textbf{68,51} & 63,82          & \textbf{69,78} & 73,90          & \textbf{81,70} & 69,97          \\
			CORAL    & 62,71          & 80,43          & 59,52          & 49,45          & 66,30          & 78,21          & 73,63          & 63,40          & 62,98          & 63,19          & 84,67          & 74,46          & 64,85          \\
			JGSA     & 70,30          & 80,80          & 60,65          & 53,85          & \textbf{79,35} & 68,69          & 66,48          & 66,16          & 63,68          & 53,85          & 75,83          & 81,52          & 67,59          \\ \hline
			MAX      & 70,86          & 83,88          & 61,00          & 72,53          & 79,35          & 79,76          & 75,82          & 68,51          & 64,39          & 69,78          & 84,81          & 81,70          &                \\ \hline
		\end{tabular}
	}
\end{table*}



\begin{table*}[ht!]
	\centering
	\caption{Accuracy Using L2 Norm}
	\label{tab2}
	%\tabcolsep=0.06cm
	\scalebox{0.95}{
		\begin{tabular}{cccccccccccccc}
			\hline
			\begin{tabular}[c]{@{}c@{}}Method/\\ Src-Tgt\end{tabular} & AR-GX          & AR-GA          & AR-MS          & GX-AR          & GX-GA          & GX-MS          & GA-AR          & GA-GX          & GA-MS          & MS-AR          & MS-GX          & MS-GA          & Mean           \\ \hline
			NA       & 62,98          & 78,26          & 59,31          & 50,00          & 65,04          & 78,56          & 73,08          & 63,12          & 62,20          & 68,13          & 85,64          & 74,64          & 66,58          \\
			TCA      & 69,06          & \textbf{82,25} & 60,51          & 60,99          & 77,36          & 68,69          & 67,03          & 64,92          & 62,98          & 63,19          & 74,03          & 79,89          & 67,86          \\
			GFK      & 69,89          & 68,84          & 55,78          & 62,09          & 66,67          & 81,66          & 67,58          & 60,50          & 59,17          & 74,18          & \textbf{87,15} & 73,73          & 68,21          \\
			SA       & 67,82          & 66,85          & 53,81          & \textbf{71,98} & 76,81          & \textbf{82,09} & 73,08          & 63,95          & 63,19          & 70,33          & 85,77          & 77,90          & 71,15          \\
			JDA      & 69,89          & 82,07          & 60,08          & 61,54          & 77,36          & 68,41          & 67,03          & 66,85          & 63,19          & 65,38          & 73,90          & 79,71          & 67,72          \\
			TJM      & 70,17          & 80,80          & 61,00          & 71,43          & 78,44          & 68,12          & 69,78          & \textbf{68,51} & \textbf{63,82} & 69,78          & 73,90          & \textbf{81,70} & 69,97          \\
			CORAL    & 62,15          & 70,11          & 52,54          & 54,95          & 68,12          & 81,81          & 62,64          & 57,04          & 54,02          & \textbf{75,82} & 87,02          & 70,83          & 65,38          \\
			JGSA     & \textbf{70,44} & 81,70          & \textbf{61,14} & 55,49          & \textbf{79,89} & 78,84          & \textbf{74,73} & 65,88          & 63,68          & 57,14          & 84,12          & 76,81          & \textbf{72,58} \\ \hline
			MAX      & 70,44          & 82,25          & 61,14          & 71,98          & 79,89          & 82,09          & 74,73          & 68,51          & 63,82          & 75,82          & 87,15          & 81,70          &                \\ \hline
		\end{tabular}
	}
\end{table*}



\begin{table*}[ht!]
	\centering
	\caption{Accuracy Using L1 Norm - Z-score}
	\label{tab3}
	%\tabcolsep=0.06cm
	\scalebox{0.95}{
		\begin{tabular}{cccccccccccccc}
			\hline
			\begin{tabular}[c]{@{}c@{}}Method/\\ Src-Tgt\end{tabular} & AR-GX          & AR-GA          & AR-MS          & GX-AR          & GX-GA          & GX-MS          & GA-AR          & GA-GX          & GA-MS          & MS-AR          & MS-GX          & MS-GA          & Mean           \\ \hline
			NA       & 66,30          & \textbf{78,80} & 63,75          & 65,38          & 66,67          & 81,38          & 69,78          & 61,74          & 65,16          & 69,78          & \textbf{85,50} & \textbf{78,44} & 68,22          \\
			TCA      & 69,48          & 75,91          & 66,01          & 68,13          & 74,82          & 82,02          & 76,92          & 66,16          & 68,90          & \textbf{73,08} & 84,94          & 77,54          & \textbf{73,95} \\
			GFK      & 63,81          & 74,46          & 58,53          & 66,48          & 73,91          & 83,50          & \textbf{78,02} & 65,19          & 64,10          & 72,53          & 84,94          & 77,90          & 73,22          \\
			SA       & 61,74          & 74,09          & 57,05          & 64,84          & 71,38          & \textbf{83,71} & 75,82          & 67,96          & 65,73          & 72,53          & 84,12          & 76,63          & 71,95          \\
			JDA      & 58,70          & 72,64          & 62,69          & 66,48          & 78,08          & 79,83          & 77,47          & 63,54          & 68,41          & 70,33          & 85,22          & 76,09          & 71,49          \\
			TJM      & 62,02          & 73,55          & 64,74          & 64,84          & \textbf{78,44} & 80,39          & 75,82          & 63,81          & \textbf{69,89} & 69,23          & 84,94          & 77,17          & 71,72          \\
			CORAL    & 63,12          & 72,46          & 61,21          & 64,29          & 72,64          & 82,30          & 73,08          & 65,33          & 63,26          & 70,88          & 84,81          & 76,45          & 71,67          \\
			JGSA     & \textbf{76,52} & 65,58          & \textbf{71,65} & \textbf{70,88} & 76,81          & 73,70          & 63,19          & \textbf{69,48} & 61,35          & 63,74          & 75,83          & 68,12          & 70,18          \\ \hline
			MAX      & 76,52          & 78,80          & 71,65          & 70,88          & 78,44          & 83,71          & 78,02          & 69,48          & 69,89          & 73,08          & 85,50          & 78,44          &                \\ \hline
		\end{tabular}
	}
\end{table*}


\begin{table*}[ht!]
	\centering
	\caption{Accuracy Using L2 Norm - Z-score}
	\label{tab4}
	%\tabcolsep=0.06cm
	\scalebox{0.95}{
		\begin{tabular}{cccccccccccccc}
			\hline
			\begin{tabular}[c]{@{}c@{}}Method/\\ Src-Tgt\end{tabular} & AR-GX          & AR-GA          & AR-MS          & GX-AR          & GX-GA          & GX-MS          & GA-AR          & GA-GX          & GA-MS          & MS-AR          & MS-GX          & MS-GA          & Mean           \\ \hline
			NA       & 66,16          & \textbf{79,17} & 63,82          & 67,03          & 66,85          & 81,31          & 69,78          & 61,60          & 65,16          & 69,78          & \textbf{85,64} & \textbf{78,44} & 68,41          \\
			TCA      & \textbf{69,75} & 75,36          & 69,18          & \textbf{68,13} & 75,00          & 82,09          & 76,92          & 66,30          & 68,62          & \textbf{73,63} & 85,08          & 77,72          & \textbf{74,31} \\
			GFK      & 62,85          & 74,28          & 58,46          & 66,48          & 73,91          & 83,50          & \textbf{78,02} & 65,47          & 64,95          & 72,53          & 85,08          & 77,54          & 73,22          \\
			SA       & 61,46          & 73,91          & 56,98          & 64,84          & 71,74          & \textbf{83,64} & 76,37          & \textbf{67,54} & 65,66          & 72,53          & 84,53          & 76,81          & 72,13          \\
			JDA      & 61,33          & 71,56          & 62,83          & 66,48          & 77,54          & 79,27          & 77,47          & 66,30          & 68,55          & 70,33          & 84,94          & 75,18          & 70,94          \\
			TJM      & 61,88          & 73,91          & 64,74          & 64,84          & 77,90          & 80,25          & 74,73          & 63,67          & 70,03          & 69,23          & 84,81          & 77,54          & 71,97          \\
			CORAL    & 63,40          & 72,10          & 61,07          & 64,29          & 72,46          & 82,37          & 73,63          & 64,23          & 63,82          & 69,78          & 85,08          & 76,81          & 70,94          \\
			JGSA     & 54,01          & 65,76          & \textbf{71,37} & 64,84          & \textbf{81,52} & 72,92          & 51,10          & 67,13          & \textbf{71,93} & 68,68          & 72,24          & 72,46          & 70,02          \\ \hline
			MAX      & 69,75          & 79,17          & 71,37          & 68,13          & 81,52          & 83,64          & 78,02          & 67,54          & 71,93          & 73,63          & 85,64          & 78,44          &                \\ \hline
		\end{tabular}
	}
\end{table*}

\fi

% 1) Resultados medios maiores podem indicar a estabilidade sobre diferentes combinações de domain adaptation

% 2) A diferença de conhecimento que pode ser extraido de um dominio I(A;B)==I(B;A) mas E(A|B) << E(B|A),i.e a incerteza de A dado que B é conhecido é menor do que a incerteza de B dado que A é conhecido 

% 3) Negative transfer... temos as opções onde, o processamento se fez perder informação, ou mesmo que algum método na teoria tenha colocado a informação mais facil de ser extraida o classificador nao obteve exito

% Run all experiments again over all possible parameters (will take 12hr+)

\iffalse

\begin{table*}[]
	\centering
	\caption{Positive (blue) and Negative (red) Transfer using L2 Norm - Z-score}
	\label{tab5}
	%\tabcolsep=0.06cm
	\scalebox{1.00}{
		\begin{tabular}{ccccccccccccc}
			\hline
			\begin{tabular}[c]{@{}c@{}}Method/\\ Src-Tgt\end{tabular} & AR-GX                                                & AR-GA                         & AR-MS                         & GX-AR                         & GX-GA                         & GX-MS                         & GA-AR                         & GA-GX                         & GA-MS                         & MS-AR                         & MS-GX                         & MS-GA                         \\ \hline
			NA       & 66,16                                                & 79,17                         & 63,82                         & 67,03                         & 66,85                         & 81,31                         & 69,78                         & 61,60                         & 65,16                         & 69,78                         & 85,64                         & 78,44                         \\
			TCA      & \color{blue} 69,75 & \color{red}75,36 & \color{blue}69,18 & \color{blue}68,13 & \color{blue}75,00 & \color{blue}82,09 & \color{blue}76,92 & \color{blue}66,30 & \color{blue}68,62 & \color{blue}73,63 & \color{red}85,08 & \color{red}77,72 \\
			GFK      & \color{red}62,85                        & \color{red}74,28 & \color{red}58,46 & \color{red}66,48 & \color{blue}73,91 & \color{blue}83,50 & \color{blue}78,02 & \color{blue}65,47 & \color{red}64,95 & \color{blue}72,53 & \color{red}85,08 & \color{red}77,54 \\
			SA       & \color{red}61,46                        & \color{red}73,91 & \color{red}56,98 & \color{red}64,84 & \color{blue}71,74 & \color{blue}83,64 & \color{blue}76,37 & \color{blue}67,54 & \color{blue}65,66 & \color{blue}72,53 & \color{red}84,53 & \color{red}76,81 \\
			JDA      & \color{red}61,33                        & \color{red}71,56 & \color{red}62,83 & \color{red}66,48 & \color{blue}77,54 & \color{red}79,27 & \color{blue}77,47 & \color{blue}66,30 & \color{blue}68,55 & \color{blue}70,33 & \color{red}84,94 & \color{red}75,18 \\
			TJM      & \color{red}61,88                        & \color{red}73,91 & \color{blue}64,74 & \color{red}64,84 & \color{blue}77,90 & \color{red}80,25 & \color{blue}74,73 & \color{blue}63,67 & \color{blue}70,03 & \color{red}69,23 & \color{red}84,81 & \color{red}77,54 \\
			CORAL    & \color{red}63,40                        & \color{red}72,10 & \color{red}61,07 & \color{red}64,29 & \color{blue}72,46 & \color{blue}82,37 & \color{blue}73,63 & \color{blue}64,23 & \color{red}63,82 & \color{red}69,78 & \color{red}85,08 & \color{red}76,81 \\
			JGSA     & \color{red}54,01                        & \color{red}65,76 & \color{blue}71,37 & \color{red}64,84 & \color{blue}81,52 & \color{red}72,92 & \color{red}51,10 & \color{blue}67,13 & \color{blue}71,93 & \color{red}68,68 & \color{red}72,24 & \color{red}72,46 \\ \hline
		\end{tabular}
	}
\end{table*}

\fi

\begin{table*}[]
	\centering
	\caption{Positive (blue) and Negative (red) Transfer using L2 Norm - Z-score}
	\label{tab5}
	\begin{tabular}{cccccccccccccc}
		\hline
		\begin{tabular}[c]{@{}c@{}}Method /\\ Src-Tgt\end{tabular} & AR-GX & AR-GA & AR-MS & GX-AR & GX-GA & GX-MS & GA-AR & GA-GX & GA-MS & MS-AR & MS-GX & MS-GA & Mean  \\ \hline
		NA                                                         & 66,16 & 79,17 & 63,82 & 67,03 & 66,85 & 81,31 & 69,78 & 61,60 & 65,16 & 69,78 & 85,64 & 78,44 & 68,41 \\
		TCA                                                        & \color{blue}69,75 & \color{red}75,36 & \color{blue}69,18 & \color{blue}68,13 & \color{blue}75,00 & \color{blue}82,09 & \color{blue}76,92 & \color{blue}66,30 & \color{blue}68,62 & \color{blue}73,63 & \color{red}85,08 & \color{red}77,72 & 74,31 \\
		GFK                                                        & \color{red}62,85 & \color{red}74,28 & \color{red}58,46 & \color{red}66,48 & \color{blue}73,91 & \color{blue}83,50 & \color{blue}78,02 & \color{blue}65,47 & \color{red}64,95 & \color{blue}72,53 & \color{red}85,08 & \color{red}77,54 & 73,22 \\
		SA                                                         & \color{red}61,46 & \color{red}73,91 & \color{red}56,98 & \color{red}64,84 & \color{blue}71,74 & \color{blue}83,64 & \color{blue}76,37 & \color{blue}67,54 & \color{blue}65,66 & \color{blue}72,53 & \color{red}84,53 & \color{red}76,81 & 72,13 \\
		JDA                                                        & \color{red}61,33 & \color{red}71,56 & \color{red}62,83 & \color{red}66,48 & \color{blue}77,54 & \color{red}79,27 & \color{blue}77,47 & \color{blue}66,30 & \color{blue}68,55 & \color{blue}70,33 & \color{red}84,94 & \color{red}75,18 & 70,94 \\
		TJM                                                        & \color{red}61,88 & \color{red}73,91 & \color{blue}64,74 & \color{red}64,84 & \color{blue}77,90 & \color{red}80,25 & \color{blue}74,73 & \color{blue}63,67 & \color{blue}70,03 & \color{red}69,23 & \color{red}84,81 & \color{red}77,54 & 71,97 \\
		CORAL                                                      & \color{red}63,40 & \color{red}72,10 & \color{red}61,07 & \color{red}64,29 & \color{blue}72,46 & \color{blue}82,37 & \color{blue}73,63 & \color{blue}64,23 & \color{red}63,82 & \color{red}69,78 & \color{red}85,08 & \color{red}76,81 & 70,94 \\
		JGSA                                                       & \color{red}54,01 & \color{red}65,76 & \color{blue}71,37 & \color{red}64,84 & \color{blue}81,52 & \color{red}72,92 & \color{red}51,10 & \color{blue}67,13 & \color{blue}71,93 & \color{red}68,68 & \color{red}72,24 & \color{red}72,46 & 70,02 \\ \hline
	\end{tabular}
\end{table*}



\subsection{Complementariness of Cross-Domain Predictions}

In this subsection, we select the pair (l2-Norm-Z-score/TCA) to analyse the complementariness of predictions between source and target data. Given a target data each group from the diagram represents a source data which the pair (l2-Norm-Z-score/TCA) was trained and afterwards test on target data. 
The intersections between sets show samples that were predicted correctly by both sets. The results were represented in Venn diagrams, which are shown in Figure \ref{fig:venn}.

\begin{figure}[h!]
	\centering
	\subfloat[Arceburgo]{
		\includegraphics[width=0.5\columnwidth]{pdf/venn_tgt_arceburgo.pdf}
		\label{fig:fig1}
	}
	\subfloat[Guaxup\'{e}]{
		\includegraphics[width=0.5\columnwidth]{pdf/venn_tgt_guaxupe.pdf}
		\label{fig:fig2}
	}
	
	\subfloat[Guaran\'{e}sia]{
		\includegraphics[width=0.5\columnwidth]{pdf/venn_tgt_guaranesia.pdf}
		\label{fig:fig3}
	}
	\subfloat[Montesanto]{
		\includegraphics[width=0.5\columnwidth]{pdf/venn_tgt_montesanto.pdf}
		\label{fig:fig4}
	}
	\caption{Veen diagram for samples correctly predicted in different target data, where the intersections between sets shows samples that were predicted correctly by both sets. Target data: \textbf{(a)} Arceburgo. \textbf{(b)} Guaxup\'{e}. \textbf{(c)} Guaranesia. \textbf{(d)} Monte Santo.}
	\label{fig:venn}
\end{figure}

As expected, most of the samples in all diagrams are at the intersection of three sets, i.e., the easiest samples are correctly predicted if trained in any of the available source datasets. However, in all cases it is possible to notice a considerable number of samples that were correctly predicted only from a single source, e.g., at Figure \ref{fig:fig2} a model trained in Montesanto is capable to correctly predict 110 samples not in common which the models trained in Arceburgo or Guaran\'{e}sia. This suggests the existence of complementary information that can be exploited to build a more reliable learning model.\note{Usar acronimos MS,AR e GA ?}
It is also noticeable a relationship of ``similarity'' between domains. That is, some pair of domains perform better than others, for instance, Guaxup\'{e} and Montesanto, in Figure \ref{fig:fig2} a model trained in Montesanto and in Figure \ref{fig:fig4} a model trained in Guaxup\'{e}. However, this relationship is not always bidirectional, for example, the case of Arceburgo and Guaran\'{e}sia, in Figure \ref{fig:fig1} Guaran\'{e}sia perform well as a source domain, predicting correctly 140 over 182 (76,92\%) samples, but in Figure \ref{fig:fig3} Montesanto is more useful than Arceburgo, predicting correctly 429 over 552 (77,71\%) samples in a comparison of 416 (75,36\%) from Arceburgo.

\subsection{Visual Analysis}

%\msa{The following sentence is too long. Break it into smaller sentences, and try to make them clearer.}
%\sout{Motivated by the samples correctly predicted (and shown in Venn Diagrams \ref{fig:venn}), in this section we investigate the spatial relationship between these samples but considering only these outside the intersections between models, i.e., given a fix adaptation approach, we are focusing on samples that were correctly predicted exclusively for that source data in specific.}
%Motivated by the samples correctly predicted (and shown in Venn Diagrams \ref{fig:venn}), 
In this section we investigate the spatial relationship among the samples. Given a fix adaptation approach, we are focusing on samples that were correctly predicted exclusively for that source data in specific. For this purpose, we propose a visual analysis of these samples using two different methods to project the original representation of data in 2D-space: Principal Component Analysis and t-Distributed Stochastic Neighbor Embedding (TSNE). The projections from PCA and TSNE data are showed in Figure \ref{fig:complement_pca} and \ref{fig:complement_tsne} respectively.

\begin{figure}[]
	\centering
	\subfloat[Arceburgo]{
		\includegraphics[width=0.48\columnwidth]{pdf/complementary_arceburgo.pdf}
	}
	\subfloat[Guaxup\'{e}]{
		\includegraphics[width=0.48\columnwidth]{pdf/complementary_guaxupe.pdf}
	}

	\subfloat[Guaran\'{e}sia]{
		\includegraphics[width=0.48\columnwidth]{pdf/complementary_guaranesia.pdf}
	}
	\subfloat[Montesanto]{
		\includegraphics[width=0.48\columnwidth]{pdf/complementary_montesanto.pdf}
	}
	\caption{2D-Space Projections using PCA}
	\label{fig:complement_pca}
\end{figure}

\begin{figure}[]
	\centering
	\subfloat[Arceburgo]{
		\includegraphics[width=0.48\columnwidth]{pdf/complementary_TSNEarceburgo.pdf}
	}
	\subfloat[Guaxup\'{e}]{
		\includegraphics[width=0.48\columnwidth]{pdf/complementary_TSNEguaxupe.pdf}
	}
	
	\subfloat[Guaran\'{e}sia]{
		\includegraphics[width=0.48\columnwidth]{pdf/complementary_TSNEguaranesia.pdf}
	}
	\subfloat[Montesanto]{
		\includegraphics[width=0.48\columnwidth]{pdf/complementary_TSNEmontesanto.pdf}
	}
	\caption{2D-Space Projections using TSNE}
	\label{fig:complement_tsne}
\end{figure}


%\msa{Also the following paragraph is quite confusing! A through revision is needed.}
%With a visual analysis of the projections it is possible to notice \note{optional} important aspects of data and the complementariness between source data. Firstly, PCA projections do not show much insight about spatial relationship of correctly predicted samples; instead it shows some sparsity over the features space. The PCA projection is a powerful dimensional reduction technique since it projects the original high-dimensional data to directions with preserve the maximum variance as possible, however, the local structure of original data is not preserved, i.e., points that are close, regarding to some metric, in original high dimensional space do not remain close in the new low-dimensional space. Secondly, in contrast with PCA, TSNE using a non-linear manifold approach can successfully create a low-dimensional representations preserving local structures, as can be seen in Figure \ref{fig:complement_tsne}. In addition, we can notice a leaning of a complementariness between learning models, since the samples corrected predict from different sources are tending to create clusters. This behavior in projections can be a suggestive interpretation of shared properties between the source and target data where the clusters show samples whose are more likely to be drawn from a specific source data. Another way of seeing the previous interpretation is taking in consideration the fact of remote sensing images normally can present a high intra-class variance due to the huge spatial extension explored, where an entire image can be seen as a composition of several probabilities distributions which some of them are better explained from different sources data.

With a visual analysis of the projections, it is possible to notice important aspects of data and the complementariness between source data. First, PCA projections show little insight into the spatial relationship of correctly predicted samples; instead, it shows sparsity over the features space. The PCA projection is a powerful dimensional reduction technique since it projects the original high-dimensional data in a low-dimensional space preserving the maximum variance as possible. However, PCA not preserve the local structure of original data, i.e., points that are close, regarding some metric, in original high-dimensional space do not remain close in the new low-dimensional space. Second, in contrast with PCA, TSNE using a non-linear manifold approach can successfully create a low-dimensional representations preserving local structures, as shown in Figure \ref{fig:complement_tsne}. In addition, we can notice a leaning of a complementariness between learning models, since the samples corrected predict from different sources are tending to create clusters. This behavior in projections can be a suggestive interpretation of shared properties between the source and target data where the clusters show samples whose are more likely to be drawn from a specific source data. Another way of seeing the previous interpretation is taking in consideration the fact of remote sensing images can present a high intra-class variance due to the huge spatial extension explored. An entire image can be seen as a composition of several probabilities distributions which some of them are better explained from different sources of data.



%"The first step around any data related challenge is to start by exploring the data itself. This could be by looking at, for example, the distributions of certain variables or looking at potential correlations between variables.

%The problem nowadays is that most datasets have a large number of variables. In other words, they have a high number of dimensions along which the data is distributed. Visually exploring the data can then become challenging and most of the time even practically impossible to do manually. However, such visual exploration is incredibly important in any data-related problem. Therefore it is key to understand how to visualise high-dimensional datasets. This can be achieved using techniques known as dimensionality reduction. This post will focus on two techniques that will allow us to do this: PCA and t-SNE."




\iffalse
%%% Resultados com a avaliação no proprio dataset
\begin{table}[]
	\centering
	\caption{Data distribution}
	\label{tab0}
	\begin{tabular}{ccc}
		\hline
		Num Samples    & Non-Coffee (Balanced) & Coffee \\ \hline
		Arceburgo(AR)  & 5.004 (91)            & 91     \\
		Guaran\'{e}sia(GA) & 276 (276)             & 276    \\
		Guaxupe(GX)    & 6.825 (362)           & 362    \\
		Montesanto(MS) & 15.384 (709)          & 709    \\ \hline
	\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{Accuracy Using L1 Norm}
\label{tab1}
\tabcolsep=0.09cm
\scalebox{0.95}{
	\begin{tabular}{cccccccccccccc}
		\hline
		\begin{tabular}[c]{@{}c@{}}Method/\\ Src-Tgt\end{tabular} & AR-GX          & AR-GA          & AR-MS          & GX-AR          & GX-GA          & GX-MS          & GA-AR          & GA-GX          & GA-MS          & MS-AR          & MS-GX          & MS-GA          & Mean           \\ \hline
		NA       & 63,26          & 80,62          & 59,03          & 60,44          & 77,36          & 75,67          & 70,88          & 64,64          & 63,82          & 52,20          & 79,56          & 78,44          & 67,76          \\
		TCA      & 69,06          & 82,25          & 60,51          & 60,99          & 77,36          & 68,69          & 67,03          & 64,92          & 62,98          & 63,19          & 74,03          & 79,89          & 67,86          \\
		GFK      & 68,78          & 81,88          & 60,37          & 55,49          & 71,38          & 78,77          & \textbf{75,82} & 63,95          & 62,91          & 63,19          & \textbf{84,81} & 73,91          & 70,08          \\
		SA       & \textbf{70,86} & \textbf{83,88} & 59,73          & \textbf{72,53} & 77,17          & \textbf{79,76} & 73,08          & 64,09          & \textbf{64,39} & 63,19          & 84,67          & 77,54          & \textbf{72,80} \\
		JDA      & 69,89          & 82,07          & 60,08          & 61,54          & 77,36          & 68,41          & 67,03          & 66,85          & 63,19          & 65,38          & 73,90          & 79,71          & 67,72          \\
		TJM      & 70,17          & 80,80          & \textbf{61,00} & 71,43          & 78,44          & 68,12          & 69,78          & \textbf{68,51} & 63,82          & \textbf{69,78} & 73,90          & \textbf{81,70} & 69,97          \\
		CORAL    & 62,71          & 80,43          & 59,52          & 49,45          & 66,30          & 78,21          & 73,63          & 63,40          & 62,98          & 63,19          & 84,67          & 74,46          & 64,85          \\
		JGSA     & 70,30          & 80,80          & 60,65          & 53,85          & \textbf{79,35} & 68,69          & 66,48          & 66,16          & 63,68          & 53,85          & 75,83          & 81,52          & 67,59          \\ \hline
		MAX      & 70,86          & 83,88          & 61,00          & 72,53          & 79,35          & 79,76          & 75,82          & 68,51          & 64,39          & 69,78          & 84,81          & 81,70          &                \\ \hline
	\end{tabular}
}
\end{table}



\begin{table}[]
\centering
\caption{Accuracy Using L2 Norm}
\label{tab2}
\tabcolsep=0.09cm
\scalebox{0.95}{
	\begin{tabular}{cccccccccccccc}
		\hline
		\begin{tabular}[c]{@{}c@{}}Method/\\ Src-Tgt\end{tabular} & AR-GX          & AR-GA          & AR-MS          & GX-AR          & GX-GA          & GX-MS          & GA-AR          & GA-GX          & GA-MS          & MS-AR          & MS-GX          & MS-GA          & Mean           \\ \hline
		NA       & 62,98          & 78,26          & 59,31          & 50,00          & 65,04          & 78,56          & 73,08          & 63,12          & 62,20          & 68,13          & 85,64          & 74,64          & 66,58          \\
		TCA      & 69,06          & \textbf{82,25} & 60,51          & 60,99          & 77,36          & 68,69          & 67,03          & 64,92          & 62,98          & 63,19          & 74,03          & 79,89          & 67,86          \\
		GFK      & 69,89          & 68,84          & 55,78          & 62,09          & 66,67          & 81,66          & 67,58          & 60,50          & 59,17          & 74,18          & \textbf{87,15} & 73,73          & 68,21          \\
		SA       & 67,82          & 66,85          & 53,81          & \textbf{71,98} & 76,81          & \textbf{82,09} & 73,08          & 63,95          & 63,19          & 70,33          & 85,77          & 77,90          & 71,15          \\
		JDA      & 69,89          & 82,07          & 60,08          & 61,54          & 77,36          & 68,41          & 67,03          & 66,85          & 63,19          & 65,38          & 73,90          & 79,71          & 67,72          \\
		TJM      & 70,17          & 80,80          & 61,00          & 71,43          & 78,44          & 68,12          & 69,78          & \textbf{68,51} & \textbf{63,82} & 69,78          & 73,90          & \textbf{81,70} & 69,97          \\
		CORAL    & 62,15          & 70,11          & 52,54          & 54,95          & 68,12          & 81,81          & 62,64          & 57,04          & 54,02          & \textbf{75,82} & 87,02          & 70,83          & 65,38          \\
		JGSA     & \textbf{70,44} & 81,70          & \textbf{61,14} & 55,49          & \textbf{79,89} & 78,84          & \textbf{74,73} & 65,88          & 63,68          & 57,14          & 84,12          & 76,81          & \textbf{72,58} \\ \hline
		MAX      & 70,44          & 82,25          & 61,14          & 71,98          & 79,89          & 82,09          & 74,73          & 68,51          & 63,82          & 75,82          & 87,15          & 81,70          &                \\ \hline
	\end{tabular}
}
\end{table}



\begin{table}[]
	\centering
	\caption{Accuracy Using L1 Norm - Z-score}
	\label{tab3}
	\tabcolsep=0.09cm
	\scalebox{0.95}{
	\begin{tabular}{cccccccccccccc}
		\hline
		\begin{tabular}[c]{@{}c@{}}Method/\\ Src-Tgt\end{tabular} & AR-GX          & AR-GA          & AR-MS          & GX-AR          & GX-GA          & GX-MS          & GA-AR          & GA-GX          & GA-MS          & MS-AR          & MS-GX          & MS-GA          & Mean           \\ \hline
		NA       & 66,30          & \textbf{78,80} & 63,75          & 65,38          & 66,67          & 81,38          & 69,78          & 61,74          & 65,16          & 69,78          & \textbf{85,50} & \textbf{78,44} & 68,22          \\
		TCA      & 69,48          & 75,91          & 66,01          & 68,13          & 74,82          & 82,02          & 76,92          & 66,16          & 68,90          & \textbf{73,08} & 84,94          & 77,54          & \textbf{73,95} \\
		GFK      & 63,81          & 74,46          & 58,53          & 66,48          & 73,91          & 83,50          & \textbf{78,02} & 65,19          & 64,10          & 72,53          & 84,94          & 77,90          & 73,22          \\
		SA       & 61,74          & 74,09          & 57,05          & 64,84          & 71,38          & \textbf{83,71} & 75,82          & 67,96          & 65,73          & 72,53          & 84,12          & 76,63          & 71,95          \\
		JDA      & 58,70          & 72,64          & 62,69          & 66,48          & 78,08          & 79,83          & 77,47          & 63,54          & 68,41          & 70,33          & 85,22          & 76,09          & 71,49          \\
		TJM      & 62,02          & 73,55          & 64,74          & 64,84          & \textbf{78,44} & 80,39          & 75,82          & 63,81          & \textbf{69,89} & 69,23          & 84,94          & 77,17          & 71,72          \\
		CORAL    & 63,12          & 72,46          & 61,21          & 64,29          & 72,64          & 82,30          & 73,08          & 65,33          & 63,26          & 70,88          & 84,81          & 76,45          & 71,67          \\
		JGSA     & \textbf{76,52} & 65,58          & \textbf{71,65} & \textbf{70,88} & 76,81          & 73,70          & 63,19          & \textbf{69,48} & 61,35          & 63,74          & 75,83          & 68,12          & 70,18          \\ \hline
		MAX      & 76,52          & 78,80          & 71,65          & 70,88          & 78,44          & 83,71          & 78,02          & 69,48          & 69,89          & 73,08          & 85,50          & 78,44          &                \\ \hline
	\end{tabular}
}
\end{table}


\begin{table}[]
\centering
\caption{Accuracy Using L2 Norm - Z-score}
\label{tab4}
\tabcolsep=0.09cm
\scalebox{0.95}{
	\begin{tabular}{cccccccccccccc}
		\hline
		\begin{tabular}[c]{@{}c@{}}Method/\\ Src-Tgt\end{tabular} & AR-GX          & AR-GA          & AR-MS          & GX-AR          & GX-GA          & GX-MS          & GA-AR          & GA-GX          & GA-MS          & MS-AR          & MS-GX          & MS-GA          & Mean           \\ \hline
		NA       & 66,16          & \textbf{79,17} & 63,82          & 67,03          & 66,85          & 81,31          & 69,78          & 61,60          & 65,16          & 69,78          & \textbf{85,64} & \textbf{78,44} & 68,41          \\
		TCA      & \textbf{69,75} & 75,36          & 69,18          & \textbf{68,13} & 75,00          & 82,09          & 76,92          & 66,30          & 68,62          & \textbf{73,63} & 85,08          & 77,72          & \textbf{74,31} \\
		GFK      & 62,85          & 74,28          & 58,46          & 66,48          & 73,91          & 83,50          & \textbf{78,02} & 65,47          & 64,95          & 72,53          & 85,08          & 77,54          & 73,22          \\
		SA       & 61,46          & 73,91          & 56,98          & 64,84          & 71,74          & \textbf{83,64} & 76,37          & \textbf{67,54} & 65,66          & 72,53          & 84,53          & 76,81          & 72,13          \\
		JDA      & 61,33          & 71,56          & 62,83          & 66,48          & 77,54          & 79,27          & 77,47          & 66,30          & 68,55          & 70,33          & 84,94          & 75,18          & 70,94          \\
		TJM      & 61,88          & 73,91          & 64,74          & 64,84          & 77,90          & 80,25          & 74,73          & 63,67          & 70,03          & 69,23          & 84,81          & 77,54          & 71,97          \\
		CORAL    & 63,40          & 72,10          & 61,07          & 64,29          & 72,46          & 82,37          & 73,63          & 64,23          & 63,82          & 69,78          & 85,08          & 76,81          & 70,94          \\
		JGSA     & 54,01          & 65,76          & \textbf{71,37} & 64,84          & \textbf{81,52} & 72,92          & 51,10          & 67,13          & \textbf{71,93} & 68,68          & 72,24          & 72,46          & 70,02          \\ \hline
		MAX      & 69,75          & 79,17          & 71,37          & 68,13          & 81,52          & 83,64          & 78,02          & 67,54          & 71,93          & 73,63          & 85,64          & 78,44          &                \\ \hline
	\end{tabular}
}
\end{table}

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Discussion}

%Authors should discuss the results and how they can be interpreted in perspective of previous studies and of the working hypotheses. The findings and their implications should be discussed in the broadest context possible. Future research directions may also be highlighted.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








==> tex/Introduction_edemir.tex <==
\section{Introduction}\label{intro}

\iffalse
\begin{itemize}
	\color{red}
	\item Grande quantidade de dados provenientes de sensores são gerados levando a uma grande quantidade de dados a serem analisados.
	
	\item Apesar da quantidade de dados gerados, a escassez de dados rotulados ainda é um problema principalmente nas abordagens de visão computacional onde se é usado a aprendizagem supervisionada
		
	\item Para contornar esse caso, a adaptação de domínio não supervisionada é usada.
	
	\item Uma das grandes motivações em relação a adaptação de domínio é na área de sensoriamento remoto (discursar o porque em sensoriamento remoto a adaptação de domínio é muito importante)
	
	\item O que foi está sendo proposto no paper, como isso foi feito e a descrição das próximas seções.
\end{itemize}

\fi

%The introduction should briefly place the study in a broad context and highlight why it is important. It should define the purpose of the work and its significance.
%\jef{Frase començando com verbo? Quem ``aumentou''? REESCREVER!}

%Over the years, there has increased significantly \note{optional} the number of remote sensing images availability.
%This was possible thanks to a new generation of satellite missions with short revisit time, as well the popular commercialization of drone-mounted cameras~\cite{tuia2016domain}.
The accessibility to large sets of remote sensing images has increased over the years. The main reasons are a new generation of satellite missions with short revisit time, as well as the popularization of drone mounted cameras.

Despite the extensive quantity of unlabeled data for visual analysis, a lack of labeled data is still a problem for some applications in remote sensing. This normally happens because of the difficult to acquire or create labeled sets. For example, in agriculture is common to send specialists to the field to collect and identify the data. Considering that a large scale plantation can cover hundreds of kilometers, a manual inspection over the area can last more than months and be finishing obtaining annotations \note{data} with a difference of dates. Another obstacle is the bad accessibility of the interested region. Depending on the application, is expensive or even impossible to recollect the required labeled data and rebuild learning models for every new task. Since the annotated data is essential for a good performance of supervised learning methods, alternative ways are explored.

%\note{Desenvolver o problema de falta de dados anotados: ;como isso pode afetar; como é feito atualmente, ; porque isso é um problema}
To surpass the problem, several approaches were developed in the last years, exploiting unlabeled data in concern of unsupervised domain adaptation (UDA). In this manner, labeled data can be employed from one or more prior datasets with the aim of create a learning model for unseen or unlabeled data.
%\jef{SIM! O que é adaptação de domínio? Como isso pode ajudar a solucionar o problema que você mencionou? Minha sugestão é você discutir do ponto de vista conceitual que bases de conhecimento já existentes podem formar uma rede. Talvez seja interessante criar uma figura.}
%In general, the \note{The} unsupervised domain adaptation problem takes advantage of labeled data in one or more source domains with the objective \note{aim} of create a learning model for unseen or unlabeled data in a target domain.
% Essa parte ficou complexa e confusa.
%However, domain adaptation has the main assumption that exists an affinity between a source and target domains, but strong enough to differ from a supervised learning problem where both data originate from the same distribution. 
%In other words, when \note{When} the assumption of domain adaptation is satisfied, the source and target domain distributions have related but different distributions
When the assumption of UDA is satisfied, the source (prior labeled datasets) and target (new unlabeled interested data) domain have related but different probability distributions and such divergence is named as \emph{domain shift}.
Such phenomenon can be seen in several visual applications. For example, human pose changes in estimation task, a variation of luminosity in photos, differences in acquisition sensor, multi-view descriptions of the same object (draw, sketch, photo, textual description) etc.

% Optional
%Domain shift is also present in remote sensing context, as can be seen in Figure \ref{domain_shift}.

Since supervised learning methods expect that both data follow the same distribution, domain shift can degrade the performance on target if trained directly in a source domain without a correct adaptation. In view of the challenges proposed by unsupervised domain adaptation, this research field has been drawing attention in last years due to the realistic proposed scenarios~\cite{zhangtransfer}.

%One major motivation of this paper is to handle with domain adaptation of agriculture images.
The main motivation of this letter is to handle with domain adaptation for agriculture scenarios. More specifically, we are interested in mapping coffee crops across different geographic domains, i.e., we want to evaluate if existing UDA methods are effective in scenarios with plant variations and terrain conditions. Although the use of remote sensing is crucial, the monitoring of agricultural activities shows unique challenges regarding the others computer vision applications. For instance, the coffee production follows strong seasonal patterns related to the biological life-cycle of crops. In addition, it depends on the physical landscape (e.g. soil type, elevation, etc) as well \note{and} their climatic driving variables due to the relationships with photo-period, fruits removal, photosynthesis and agricultural management practices \cite{atzberger2013advances}. Since the data is highly \note{optional} variable in space and time, a domain shift is clearly \note{optional} notable and a great effort is required to identify and make a transference of knowledge between a labeled source data to an unlabeled target domain. 

%\jef{Esse paragrafo esta meio estranho. Sugiro reescrever pra deixar a ideia mais clara.}
Unsupervised domain adaptation draw attention particularly for remote-sensing expecialists. In this field is common provide particular solutions for every new mapping and detection task. Avoiding discart labeled images available from a similar task and adapt to improve a new remote sensing task is highly desired.
%\sout{Furthermore, remote-sensing experts are exclusively interested in domain adaptation since it is common to provide particular solutions for detection/mapping tasks, discarding the previous solutions. In addition, is ignored the fact that multiple images available from a similar task could be adapted to improve a new remote sensing task.} 
However, as showed by authors in \cite{zhao2017multiple} the performance on a target domain depends on the worst empirical error among multiple source domains. So an insertion of non adaptive data without an adequate adaptation can degrade a final learning model or lead to suboptimal solutions.

%However, in many application scenarios, the labeled data available may come from multiple domains with different distributions. As a result, naive application of the single-source-single-target DA algorithms may lead to suboptimal solutions. Such problem calls for an efficient technique for multiple source domain adaptation.

%\jef{Acho que da pra reescrever e reduzir esse paragrafo pela metade.}

Encouraged by these challenges, in this paper we propose a comparative experimental study of various methods for UDA in a specific view of remote sensing data. To evaluate, we use the dataset, Brazilian Coffee Crops, that contains four remote sensing images of coffee crop agriculture in scenarios with plant variations and terrain conditions. We analyze the 7 methods through empirical studies using different ways to normalize data, inspecting the visual behavior and complementarity over the final predictions.

%In our experiments, firstly \note{optional} we study the most commons normalization methods for data processing. Thereafter, we propose an analysis of predictions from different adaptation methods and shown the complementary acknowledgment extracted from various approaches. At last a visual study was made over the samples corrected predicted from different adaptation methods, projecting in a 2D-space using two visualization approaches.

%\sout{Encouraged by these challenges, in this paper we propose a comparative experimental study of various methods for unsupervised domain adaptation in a specific view of remote sensing data. In order to \note{To} evaluate,  we use the dataset, Brazilian Coffee Crops, that contains \note{has} four remote sensing images of coffee crop agriculture in different geolocation \note{spatial context}. In our experiments, firstly \note{optional} we study the most commons normalization methods for data processing. Thereafter, we propose an analysis of predictions from different adaptation methods and shown the complementary acknowledgment extracted from various approaches. At last a visual study was made over the samples corrected predicted from different adaptation methods, projecting in a 2D-space using two visualization approaches.}


==> tex/RelatedWork_edemir.tex <==

\iffalse
\section{Background Concepts}\label{background}


\begin{itemize}
	\color{red}
		
	\item Definição formal do problema UDA (Unsupervised Domain Adaptation): Domain, Task, Dataset, Problem
	
	\item Como o problema é ramificado de acordo com as abordagens dos artigos na literatura.(data centric e subspace centric)
	
	\item Discutir as vantagens e desvantagens de todos os baselines em uma linha cronológica em que eles foram propostos, e fazer uma tabela marcando as principais vantagens-desvantagens para ficar de fácil visualização.
	
\end{itemize}

In this work we follow the definitions proposed by Zhang et~al.~\cite{zhang2017cross} for ``domain'', ``task'' and ``dataset''.

\textit{Definition 1:} A \textbf{domain} is defined as $D = \{X, P(x)\}$, which is composed of two components: a feature space X and a marginal probability distribution $P(x)$, where $x \in X$ .

\textit{Definition 2:} Given a specific domain, a \textbf{task} is defined as $T = \{Y, f(x)\}$, which is composed of two components: a label space $Y$ and a predictive function $f(x)$, where $f(x)$ can be seen as a conditional distribution $P(y|x)$ and $y \in Y$.

\textit{Definition 3:} A \textbf{dataset} is defined as $S = \{X ,P(x), Y, f(x)\}$, which is a collection of data that belong to a specific domain with a specific task.

In unsupervised domain adaptation we assume that no labeled data is available in the target dataset, i.e., the labels of target dataset are unknown, but all \note{optional} unlabeled samples are available at training phase.

With the previous \note{earlier} definitions we can state the UDA problem:

\textit{Problem:} Given labeled source domain $D_s = \{(x_1 , y_1 ), ... , (x_{n_s} , y_{n_s} )\}$ and unlabeled target domain $D_t = \{x_{1}, ... , x_{n_t}\}$, where $n_s$ and $n_t$ are number of samples in source and target domain respectively, under the assumptions that: source and target domain share the same feature and label space  ($X_s = X_t, Y_s = Y_t$), and the samples from source and target domain are drawn from different distributions but related ($P_s(x_s) \neq P_t(x_t), P_s(y_s|x_s) \neq P_t(y_t | x_t)$). How to create a function h(.) that predicts the class label of a sample from the target domain $D_t$ using labeled source domain $D_s$ and unlabeled target domain $D_t$.


The main difference between supervised learning and UDA rely on the fact we have different but related distributions between source and target, making possible to make a transference of knowledge in order \note{optional} to reduce the distribution difference between domain.

\fi

%\section{Related Work}\label{related}
\section{Unsupervised Domain Adaptation Approaches}\label{related}

%Regarding the literature \cite{zhangtransfer}, 
\jef{Continua ruim. Leia essa frase: ``UDA can be divided into three main categories of knowledge would be transferred''. O que voce quis dizer?}

%According to the literature survey [21], existing domain adaptation methods can be roughly organized into two categories: feature matching and instance reweighting

\ede{Regarding the literature \cite{zhangtransfer}, UDA methods can be organized into tree main categories}: (1) instance-based, (2) feature-based and (3) classifier-based. In instance-based adaptation is re-weight some \note{optional} data in the source domain or in both domains to reduce domain divergence. In feature representation is attempt to learn a new feature representations to minimize \note{decrease} domain shift and error of learning task. In classifier-based is learn a new model that minimizes the generalization error in the target domain via training instances from both domains.
%Since labeled data in the target domain is not available in unsupervised domain adaptation, the classifier-based adaptation is unfeasible.
%Regarding the literature, domain adaptation can be divided into three main categories of knowledge would be transferred: instance-based adaptation (re-weight some \note{optional} data in the source domain or in both domains to reduce domain divergence), feature representation adaptation (learn a new feature representations to minimize \note{decrease} domain shift and error of learning task), and classifier-based adaptation (learn a new model that minimizes the generalization error in the target domain via training instances from both domains) \cite{zhangtransfer}. Since labeled data in the target domain is not available in unsupervised domain adaptation, the classifier-based adaptation is unfeasible.
In this work, we study methods based on a feature representation category, which can be divided into three branches: Data-centric, Subspace centric, and Hybrid methods.

\subsection{Data centric Approaches}

To align a source and target data, the data-centric methods attempt find a specific transformation that can project both domains into a domain invariant space. In this way is reduced the distributional divergence between domains and preserve the data properties in original spaces. The methods in \cite{pan2011domain}, \cite{long2013transfer} and \cite{long2014transfer} are examples of data-centric approaches. In \cite{pan2011domain}, the authors proposed a method called Transfer Component Analysis (TCA) which has as objective \note{aim} learn a set of transfer components in a Reproducing Kernel Hilbert Space. When projecting domain data onto the latent space spanned by the transfer components, the distance between different distributions across domains is reduced and the variance is preserved.% as much as possible.

%Due to several external factors and noise in observation data is reliable to state that $P_s(X_s) \ne P_t(X_t)$, however TCA rely in a claim that exists a transformation $\phi$ such that $P(\phi(X_s)) \approx P(\phi(X_t))$ and $P(Y_s|\phi(X_s)) \approx P(Y_t|\phi(X_t))$. Then without the labeled data from target domain, TCA learn the transformation function $\phi$ such that: minimize the marginal distribution between $P(\phi(X_s))$ and $P(\phi(X_t))$ and preserve the variance information of the original source $X_s$ and target $X_t$ data. The both requirements remark as important for a classification task, and the Fig \ref{tca} shows solid disadvantages when these features are optimized apart.

%
%\begin{figure*}[!ht]
%	\centering
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/A.pdf}
%		\label{fig:A}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/C.pdf}
%		\label{fig:C}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/B.pdf}
%		\label{fig:B}
%	}
	
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/D.pdf}
%		\label{fig:D}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/E.pdf}
%		\label{fig:E}
%	}
%	\subfloat[]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/F.pdf}
%		\label{fig:F}
%	}
%	\caption{Importance of simultaneous optimization considering the distance of distributions and preserving the maximum variance. In \textbf{(a)} the source and target domain are clearly apart each other. Minimizing the distance between domains projecting the data over the axis $X_2$ \textbf{(b)} result in a mixture of classes degrading classification performance. However projecting the data in axis $X_1$ \textbf{(c)}, preserve variance and result in a better separability for a classification task. On the other hand, considerer the source and target domain in \textbf{(d)}. Minimizing the distance between domains in \textbf{(d)}, projecting in $X_2$ axis \textbf{(f)}, creates a good separability. While preserving the variance in $X_1$ \textbf{(e)} axis, mix and reduce discrimination of classes.}

	%\caption{Importance of simultaneous optimization considering the distance of distributions and preserving the maximum variance. In \textbf{(a)} the source and target domain are clearly apart each other. However minimizing the distance between domains projecting the data over the axis $X_2$ \textbf{(b)} result in a mixture of classes degrading classification performance, while projecting the data in axis $X_1$ \textbf{(c)}, preserve variance, result in a better separability for a classification task. On the other hand, minimizing \note{Minimizing} the distance between domains in \textbf{(d)}, projecting in $X_2$ axis \textbf{(f)}, creates a good separability while preserving the variance in $X_1$ \textbf{(e)} axis, mix and reduce discrimination of classes.}
	%Minimizing distance between marginal distributions. \textbf{(b)} Maximizing Variance.}
%	\label{tca}
%\end{figure*}

Despite TCA minimize the marginal distribution between the source and target data, the conditional distributions are not guaranteed explicit reduced in this formulation, that could lead to a poor adaptation.  To \note{In order to} handle this problem, Mingsheng et al. \cite{long2013transfer} proposed a method called Joint Distribution Adaptation (JDA) which extends the Maximum Mean Discrepancy to measure the difference in both marginal and conditional distributions. In this way JDA improve TCA, which consider only the marginal distribution, and integrate it with Principal Component Analysis to create a feature representation that is effective and robust for a large domain shift. 

%Despite TCA minimize the marginal distribution between the source and target data, the conditional distributions are not guaranteed explicit reduced in this formulation, that could lead to a poor adaptation. In order to \note{To} handle this problem, Mingsheng et al. \cite{long2013transfer} proposed a method called Joint Distribution Adaptation (JDA) which extends the Maximum Mean Discrepancy (MMD) to measure the difference in both marginal and conditional distributions (improving the TCA which consider only the marginal distribution), and integrate it with Principal Component Analysis (PCA) to create a feature representation that is effective and robust for substantial distribution difference \note{large domain shift}. To achieve this, JDA proposes a transformation T where the joint expectations of features \textbf{x} and labels \textbf{y} are matched between domains using as follows:
%\begin{equation}
%\begin{split}
%& \underset{T}{min} ||\mathbb{E}_{P(x_s, y_s)}[T(x_s), y_s] - %\mathbb{E}_{P(x_t, y_t)}[T(x_t), y_t] ||^{2} \approx \\ & %||\mathbb{E}_{P_s(x_s)}[T(x_s)] - %\mathbb{E}_{P_t(x_t)}[T(x_t)] ||^{2} + \\ & %||\mathbb{E}_{P_s(y_s|x_s)}[y_s|T(x_s)] - %\mathbb{E}_{P_t(y_t|x_t)}[y_t|T(x_t)] ||^{2}
%\end{split}
%\end{equation}
%However, since the labels in target data are not available in unsupervised domain adaptation, the $P_t(y_t|x_t)$ cannot be estimated directly. Thus JDA assumes that $P_t(y_t|x_t) \approx P_s(y_t|x_t) $ and explore the sufficient statistics of conditional distributions $P_s(x_s|y_s)$ and $P_t(x_t|y_t)$.
%where is used pseudo labels of the target data by using the predictions of a base learning model trained in source data and testing in target data.
Even when distributions between domains are minimized, some instances from source data would have more relevance than others due to the huge difference of initial data. 

%A visual example is showed in Figure \ref{tjm}.
%\begin{figure}[]
%	\centering
%	\subfloat[Aligned domains - All samples]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/Teste_Var.pdf}
%		\label{fig:Teste_Var}
%	}
%	\subfloat[Aligned domains - Relevant Samples]{
%		\includegraphics[width=0.45\columnwidth]{pdf/new/Teste_Var_2.pdf}
%		\label{fig:Teste_Var_2}
%	}
%	\label{fig:reweight}
%	\caption{The relevance of instances after a domain adaptation. An example of a source and target domains aligned is showed in \textbf{(a)}. Despite the good alignment, there is a set of samples inside the ellipse which seems to be more relevant than others (fig \textbf{b}) which recalls as outliers. Depending on learning model, irrelevant/noise samples can degrade final adaptation model highlighting the importance of reweighing the samples by their importance.}
%	\label{tjm}
%\end{figure}
To that end, a new method named Transfer Joint Matching (TJM) was proposed by Long et al. \cite{long2014transfer}. The main objective \note{aim, goal} of TJM beyond minimizing the distribution distance between domains is trying to reweigh the instances which are more valuable to a classification task in the final adaptation. 

%The Fig \ref{tjm} represents \note{is} a good example \note{intuition} of how two distributions even when adapted and aligned can show a significant difference in feature space. 
%This behavior can be exploited by focusing and reweighing the samples which are \note{optional} relevant for the adaptation. 
%Thus TJM in a two-step algorithm creates a transformation matrix T which reduce the distance of domains and reweigh the source samples to force a sparse structure between samples (Eq. \ref{tjm_opt)}).

%\begin{equation}\label{tjm_opt}
%\resizebox{\columnwidth}{!}
%{
%$\underset{T}{min} ||\mathbb{E}_{P(x_s)}[T(x_s)] - \mathbb{E}_{P(x_t)}[T(x_t)] ||^{2} + \lambda ||T||_{2,1}$
%}
%\end{equation}

%In TJM the marginal distribution is minimized through a feature matching in RKHS, as the same way of JDA, but for the reweighing of samples the authors proposed to incorporate an instance regularization in the problem formulation to force sparsity and assist in the final adaptation.

%in the transformation matrix A from Kernel-PCA, to assist in the final adaptation (Eq. \ref{sparsity}).

%\begin{equation}
%\resizebox{\columnwidth}{!}
%{
%${Sparsity~Regularization:~}
%||A_{s}||_{2,1} + ||A_{t}||_{F}^2$
%}
%\end{equation}\label{sparsity}

%Despite all mentioned methods assert that a good feature representation has to be capable of minimize the difference of distributions between domains \note{decrease the domain shift} as much as possible preserving the original properties, these methods fall in an assumption that there exists a transformation function which can project the source and target data into a common subspace which reduce the distribution difference between them and keep preserving some \note{optional} original information. Problems which a not too strongly related data \note{weak related}, i.e. strong domain shifts, can suggest that is may not exist such a space which preserve original properties and minimize in an optimal way \note{optimally} the distribution distance.

%Despite all mentioned methods assert that a good feature representation has to be capable of minimize the difference of distributions between domains \note{decrease the domain shift} as much as possible preserving the original properties, 

These methods fall in an assumption that there exists a transformation function which can project the source and target data into a common subspace which reduce the distribution difference between them and keep preserving some \note{optional} original information. Problems with a strong domain shift suggest that is may not exist such a space which preserve original properties and minimize in an optimally the distribution distance.

%Advantages of data centrics


%Disvantages of data centrics

%--However, these methods require a strong assumption that there exist a unified transformation to map source and target domains into a shared subspace with small distribution shift. [At the same time preserving the information (geometric, statistics) of the original data]

%The data centric methods only exploit shared feature in two domains, which will fail when the two different domains have large discrepancy, because there may not exist such a common space where the distributions of two domains are the same and the data properties are also maximumly preserved in the mean time.

\subsection{Subspace Centric Approaches}

By contrast of data-centric, the subspace centric methods do not assume an existence of a unified transformation but rely on a subspace manipulation of the source and target domains \cite{fernando2013unsupervised} or between them \cite{gong2012geodesic}, upholding that separate subspaces have very \note{optional} particular features to be exploited. Fernando et al. \cite{fernando2013unsupervised} propose a Subspace Alignment (SA) method, which project source and target data to different subspaces using PCA as a robust representation and learn a linear transformation matrix M that align the source subspace to the target one minimizing the Frobenius norm of their difference. In this way, the distance between different distributions across domains is reduced by moving closer the source and target subspaces exploiting the global covariance statistical structure of the two domains. 

As an alternative of subspace alignment Gong et al. \cite{gong2012geodesic} proposes an extension of the work by Gopalan et al. \cite{gopalan2011domain}, taking advantage of Grassmannian manifold. 
%In geometric definition, a Grassmannian $\mathbb{G}$(d,V) is a collection of all d-dimensional subspaces of the n-dimensional vector space V. 
%In view of domain adaptation the computed subspaces from source and target domain are mapped each one into a point in Grassmannian manifold. As pointed in \cite{gong2012geodesic}, the distance between two points in Grassmannian manifold can represent how similar the original projections are regarding their marginal distribution. %For example, consider the problem of knowledge transfer between two datasets of coffee crop in different regions of a country. The highly variable of these data, when projected into a Grassmannian manifold, will result in points far apart from each other. 
%However, the geodesic curve between these points represents intermediate subspaces which can carry some \note{optional} variant geometric and statistics properties that state a relationship between the two domains. Capture and use the largest number of subspaces as possible may help to extract the necessary information to make an effective domain adaptation.
%In \cite{gopalan2011domain} the authors explore the geodesic flow curve connecting the source and target domain on the Grassmannian manifold, sampling a discrete number of subspaces as representations and concatenation them into a feature vector for learning purpose. 
However, Gong et al. proposed the Geodesic Flow Kernel (GFK) as an elegant approach that integrates an infinite number of subspaces that lie on the geodesic flow from the source subspace to the target one using the kernel trick, and overcoming some drawbacks in the original approach. The main drawback of subspace centric methods, while focused in reducing the geometrical shift between subspaces, the distribution shift between projected data of domains are not explicitly treated as in data-centric methods, and subspace dimension to project the data normally \note{optional} require some \note{optional} tuning of parameters or preprocessing.

\subsection{Hybrid Approaches}

More recent to overcome the drawbacks of data and subspace centric methods together, Sun et al. \cite{sun2016return} propose the CORAL adaptation. In this approach, the domain shift is minimized aligning the covariance of a source and target distributions in the original data.
%For this purpose CORAL can be divided into two simple steps: 1) computation of the covariance matrices of the source and target data; 2) applying the whitening and re-coloring linear transformation only to the source features.
In contrast to the subspace centric methods, CORAL suggests an alignment without a need of subspace projection, which requires an expensive computation and hyper-parameter tuning. 
%Regarding the authors, these methods commonly \note{optional} align only the bases of subspaces, not considering the distribution of project data. 
In addition, CORAL do not assume a unified transformation such as data-centric methods, instead, the method uses an asymmetric transformation only on source data. 

In \cite{zhang2017joint} Zhang et al. propose the Joint Geometric Subspace Alignment (JGSA) that aims to reduce the statistical and geometrical divergence between domains using the common and specific properties of the source and target data. To achieve that, an overall objective function is created by taking in account five terms: target variance, a variance between/within classes, distribution shift, and subspace shift.

%To reach this objective JGSA tries to find two coupled projections A and B for source and target domain respectively that explore five different quantities together in a single objective function(Eq. \ref{jgsa}): 

%\begin{equation}
%\resizebox{\columnwidth}{!}
%{
%	$max \frac{\mu\{Target~Variance\} + \beta\{Between~Class~ Variance\} }{\{Distribution~Shift\} + \lambda\{Subspace~Shift\} + \beta\{Within~Class~Variance\}}	$
%}
%\label{jgsa}
%\end{equation}


%where $\mu$, $\lambda$, $\beta$, are regularization parameters used to handle with the trade-off of importance in every term of optimization. 

%As trying to address different drawbacks from data-centric and subspace centric, the run-time complexity of JGSA grows in comparison to the others methods since is needed to learn two different mapping projections. 

%All things considered, it seems \note{is} reasonable to assume that all methods rely on different properties covering separable challenges in UDA. Taking accounts these properties, a resume of challenges tackle for the methods is showed in Table \ref{properties}.

All methods above rely on different properties, covering separates challenges in UDA. A summary of the properties considered for each method is shown in \ref{properties}

\begin{table}[h!]
	\centering
	\caption{Comparison of Approches Properties}
	\label{properties}
\tabcolsep=0.075cm
\scalebox{0.85}
{
	\begin{tabular}{ccccccc}
		\hline
		& Approches & \begin{tabular}[c]{@{}c@{}}Preserve\\ Variance\end{tabular} & \begin{tabular}[c]{@{}c@{}}Marginal\\ Distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Conditional\\ Distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Reweight\\ Instances\end{tabular} & \begin{tabular}[c]{@{}c@{}}Geometric\\ Structure\end{tabular} \\ \hline
		\multirow{3}{*}{Data Centric} & TCA & \checkmark & \checkmark &  &  &  \\
		& JDA & \checkmark & \checkmark & \checkmark &  &  \\
		& TJM & \checkmark & \checkmark &  & \checkmark &  \\ \hline
		\multirow{2}{*}{Subspace Centric} & SA & \checkmark &  &  &  &  \\
		& GFK & \checkmark &  &  &  & \checkmark \\ \hline
		\multirow{2}{*}{Hybrid} & CORAL & \checkmark &  &  &  & \checkmark \\
		& JGSA & \checkmark & \checkmark &  & \checkmark & \checkmark \\ \hline
	\end{tabular}
}
\end{table}

